TriForecaster: A Mixture of Experts Framework for Multi-Region Electric Load Forecasting with Tri-dimensional Specialization

Electric load forecasting is pivotal for power system operation, planning and decision-making. The rise of smart grids and meters has provided more detailed and high-quality load data at multiple levels of granularity, from home to bus and cities. Motivated by similar patterns of loads across different cities in a province in eastern China, in this paper we focus on the Multi-Region Electric Load Forecasting (MRELF) problem, targeting accurate short-term load forecasting for multiple sub-regions within a large region. We identify three challenges for MRELF, including regional variation, contextual variation, and temporal variation. To address them, we propose TriForecaster, a new framework leveraging the Mixture of Experts (MoE) approach within a Multi-Task Learning (MTL) paradigm to overcome these challenges. TriForecaster features RegionMixer and Context-Time Specializer (CTSpecializer) layers, enabling dynamic cooperation and specialization of expert models across regional, contextual, and temporal dimensions. Based on evaluation on four real-world MRELF datasets with varied granularity, TriForecaster outperforms state-of-the-art models by achieving an average forecast error reduction of 22.4\%, thereby demonstrating its flexibility and broad applicability. In particular, the deployment of TriForecaster on the eForecaster platform in eastern China exemplifies its practical utility, effectively providing city-level, short-term load forecasts for 17 cities, supporting a population exceeding 110 million and daily electricity usage over 100 gigawatt-hours.

==> 1-introduction.tex <==
\section{Introduction}

% problem definition an challenges (Macro and Micro-Drift)
% case illustration
% data




% Introduce recent progress in time series forecasting and online time series forecasting. In online time series forecasting settings, the prediction model is updated with a period of data.

% However, so far, most existing online time series forecasting approaches have only targeted fitting the prediction model to historical data or the recent period of observed data. Yet, this strategy is highly restrictive, as in real-world scenarios, underlying distributions or environments of time series are constantly changing, which we call \emph{concept drift}. We divide concept drift into two categories, and Fig.x illustrates an example:

% \textbf{Macro-drift.} Macro-drift refers to stable and long-term changes in time series characteristics or patterns, which can be revealed and characterized by a period of data. For example, the power load time series shows a growth trend affected by factors such as population growth and economic development.

% \textbf{Micro-drift.}

% Moreover, the future time series might come from a new environment that is different from the historical data the model has been trained on. This requires our model to be able to understand the concept drift and further infer the future environment.

% introduction to forecasting and concept drift
% the limitations of 


Accurate time series forecasting\cite{Hyndman:forecasting:book, ACM:Survey:Deep4TSF:2022} is of great importance in many domains, such as stock market~\citep{ts:in:stock:2014,shahi2020stock}, weather~\citep{bi2023accurate}, energy~\citep{Yang:load:forecast:2023,hong2020energy}, etc. In many real-world applications, time series data arrives as a stream. It is observed that the non-stationary nature of the times series data in many scenarios makes the model trained on the historical data outdated and leads to unsatisfying forecasting on the new data~\citep{Liu2023,pham2022learning}. Thus, there is a growing interest in online time series forecasting, where the deployed model can swiftly adapt to non-stationary environments.


% Time series forecasting is of great importance in both research and applications. Accurate predictions can bring significant benefits, including traffic, weather, and electricity forecasting. Recently, there has been a Hence, there has been a considerable amount of effort dedicated to developing improved forecasting models, with attention shifting towards deep neural networks due to their ability to uncover and capture complex temporal dependencies. However, in real-world applications, there is a growing interest in the online time series forecasting scenario where the deployed model must swiftly adapt to non-stationary environments.

% In recent years, there has been significant progress in online time series forecasting. Researchers have been exploring new techniques and approaches to tackle the challenges posed by concept drift and the need for adaptive forecasting models.

% However, so far, most existing online time series forecasting approaches have only targeted fitting the prediction model to historical data or the recent period of observed data.
% However, it has been recognized that these approaches are highly restrictive, as real-world time series often exhibit \emph{concept drift}, which refers to the changing of underlying distributions or environments. 

%%However, most existing online time series forecasting approaches have primarily focused on fitting prediction models solely to historical or recent observed data, disregarding the fact that they may be evaluated on future data that can vary significantly. These approaches, however, are highly restrictive as real-world time series often exhibit \emph{concept drift}, which refers to the changing underlying distributions or environments.

Formally, in this paper, we study the \emph{concept drift} problem in time series forecasting, which refers to the changing underlying distributions or environments. 
% There are many classifications of concept drifts in times series. 
%%%{\color{blue} Most existing works classify concept drifts according to the data pattern.}  
%%%{\color{blue} However, with the development of representation learning, powerful models can easily capture patterns of these drifts. As a result, there is no necessity to design different models to capture concept drift with different data patterns. On the other hand, it is wiser to classify them according to their scope and duration of influence, and thus we can devise different learning strategies to deal with them.}
Existing taxonomies of concept drift tend to classify drifts based on data patterns. For example, in \citep{Liu2023}, the concept drift is categorized into two types: real concept drift and virtual concept drift. Other concept drift groups include sudden concept drift, incremental concept drift, gradual concept drift, and recurring concept drift~\cite{concept:drift:review:2019}. However, with the development of sophisticated representation learning techniques, these taxonomies have become less useful or sometimes misleading for modern deep learning approaches, which are capable of learning and handling these patterns easily. For example, \citep{Liu2023} defines noise occurring in time series as virtual drift, while it is not necessary for modern deep learning models as they can already learn robust time series representations against noise.

Thus, to better describe the characteristics and possible solutions for concept drifts, in this paper, we propose a new categorization into macro-drift and micro-drift for time series according to their durations. Specifically, \emph{macro-drift} refers to drifts that are stable and persist over relatively long duration. For instance, the electric power load time series exhibits a growth trend influenced by factors such as population growth and economic development. On the other hand, \emph{micro-drift} characterizes abrupt, transient changes. An example is the noticeable increase in traffic volume time series during rainy days or holidays. The different duration of the drifts calls for different learning strategies tailored to the nature of the drifts. Specifically, to address a stable macro-drift, we cannot simply apply the current optimal model to future data, as the drift itself will carry on, altering future data patterns. Therefore, we must investigate the evolution of optimal models over time and endeavor to predict the model for subsequent data. On the other hand, micro-drift is unpredictable and erratic, requiring us to monitor each incoming sample and adjust the model at test time to capture these abrupt changes. 



% Based on our forecasting practice in real-world applications, 
% in this paper, we divide it into two distinct categories, macro-drift and micro-drift, 
% as illustrated in Figure \ref{fig:concept}. 
% Specifically, \emph{macro-drift} refers to stable and long-term changes in the characteristics or patterns of time series, which can be identified and characterized by analyzing a significant period of data. For instance, the electric power load time series exhibits a growth trend influenced by factors such as population growth and economic development. On the other hand, \emph{micro-drift} refers to sudden or short-term changes in time series. Data exhibiting micro-drift may deviate from the current distribution. An example is the noticeable increase in traffic volume time series during rainy days and holidays.


 \begin{figure*}[!t]
 %\vspace{-8mm}
    \centering    
    \includegraphics[width=0.55\textwidth]{figures/LEAF-concept.pdf}
    \vspace{-3mm}
    \caption{(a) Illustration of Macro- and Micro-Drift of Time Series. (b) Design Concept of LEAF.}
    \label{fig:concept}
    \vspace{-6mm} 
\end{figure*}

% \textbf{Macro-drift.} Macro-drift refers to stable and long-term changes in time series characteristics or patterns, which can be revealed and characterized by a period of data. For example, the power load time series shows a growth trend affected by factors such as population growth and economic development.

% \textbf{Micro-drift.} Micro-drift refers to sudden or short-term changes. Data with micro-drift can be out to the current distribution. A typical example is the significant increase in traffic volume time series on rainy days and holidays.




%%Incremental and recurring concept drift in a time series forecasting  context are closely related to trends and seasonalities in the data. In particular, recurring concept drift can be easily handled by the typical handling of seasonality with dummy variables, Fourier terms and similar additional features [13]. Thus, in this study we focus on three concept drift types: sudden, incremental and gradual, which are illustrated in Figure

%%irstly, \emph{macro-drift} refers to stable and long-term changes in the characteristics or patterns of time series, which can be identified and characterized by analyzing a significant period of data. For instance, the power load time series exhibits a growth trend influenced by factors such as population growth and economic development.

%%Secondly, \emph{micro-drift} refers to sudden or short-term changes in time series. Data exhibiting micro-drift may deviate from the current distribution. An example is the noticeable increase in traffic volume time series during rainy days and holidays.




% Complicated macro and micro-drift and their superposition make it difficult for the prediction model to capture, and they keep occurring that the future time series might come from a new environment that is different from the historical data the model has been trained on. This requires our model to be able to understand the concept drift and further infer the future environment.

The research of concept drift in time series faces several challenges. Firstly, different types of concept drift, as well as their potential superposition in complex forecasting scenarios, make capturing the evolving patterns in time series data challenging. Most existing works design different strategies, e.g., historical information retrieval~\citep{arik2022self}
and fast learning~\citep{pham2022learning}, to capture concept drifts within recent observed data. However, they cannot adaptively update the model based on the influence range of drifts and ignore to adapt the model to the future data which limits the generalization ability in online time series forecasting. In particular, as many forecasting algorithms being proposed~\citep{ACM:Survey:Deep4TSF:2022}, it requires a general and versatile model-agnostic method to help them handle concept drift properly. 
Also, we notice the lack of benchmark datasets with high quality for concept drifts. 
%%%Good benchmark datasets play an important role in the advancements of the field, such as ImageNet~\citep{ImageNet:2009} for the CV field. 
%%%Although some benchmark datasets are proposed for different time series tasks, most of them are challenged for their quality~\citep{ts:dataset:survey:2023}. 
As pointed out in \citep{ts:dataset:survey:2023}, the nonstationary time series benchmark datasets are missing in the current time series benchmark datasets, which hinders the development of forecasting algorithms for concept drift. 

%Concept drifts frequently occur in real-world scenarios, making it imperative for our models to possess the capability to comprehend the concept drift phenomenon and further effectively infer the future environment.



% As it is a common practice to compare different algorithms on the benchmark datasets, and some benchmark datasets such as ImageNet~\citep{ImageNet:2009} indeed promote the advancements of these fields. 
% On the one hand, the field of time series analysis lacks benchmark datasets. On the other hand, the current limited benchmark datasets are criticized for their flaws~\citep{ts:dataset:survey:2023}. To the best of our knowledge, no widely accepted time series benchmark datasets exist for the study of concept drifts. 
% Benchmark datasets are generally used to compare different algorithms and motivate the development of new algorithms. 
%%%The next challenge lies in the difficulty of handling different types of drifts in forecasting algorithms. The presence of complex macro- and micro-drift, as well as their potential superposition, makes capturing the evolving patterns in time series data challenging. 
%%%{\color{blue} Most existing works design different strategies, e.g., historical information retrieval~\citep{arik2022self} and fast learning~\citep{pham2022learning}, to capture concept drifts within recent observed data. However, they cannot adaptively update the model based on the influence range of drifts and ignore to adapt the model to the future data which limits the generalization ability in online time series forecasting.} 
%%Concept drifts frequently occur in real-world scenarios, making it imperative for our models to possess the capability to comprehend the concept drift phenomenon and further effectively infer the future environment.

To address the concept drift problem in online time series forecasting, we propose a unified meta-learning framework called LEAF (\textbf{L}earning to \textbf{E}xtrapolate and \textbf{A}djust for \textbf{F}orecasting). LEAF is model-agnostic and can be applied to any deep prediction model, making it highly versatile. 
It learns a low-dimensional latent embedding of parameters of the target prediction model, allowing it to effectively track the dynamics of the model in response to concept drift. Optimization in the low-dimensional space conforms to the characteristics of concept drift and alleviates the over-fitting issue.
Specifically, LEAF consists of two stages: extrapolation and adjustment, to deal with macro- and micro-drift, respectively. 
In the extrapolation stage, a meta-learnt extrapolation network is employed to utilize the optimal latent embeddings from past periods and infer the latent embedding for the next period. This enables LEAF to capture and anticipate the macro-drift.
In the adjustment stage, to handle micro-drift with diverse types and extensions, we introduce a meta-learnable surrogate loss for each sample, which guides the adjustment of inferred latent embedding above to become sample-specific ones. This empowers the model to capture micro-drift patterns accurately.
In particular, we also provide theoretical analysis to justify our two-stage framework under two mild conditions. 
%%%By learning to extrapolate and adjust, the proposed LEAF framework offers a promising solution to overcome the challenges posed by concept drift in online time series forecasting, providing improved forecasting accuracy in dynamic and evolving environments.
% The proposed LEAF framework offers a promising solution to overcome the challenges posed by concept drift in online time series forecasting. By learning to extrapolate and adjust, LEAF enhances the forecasting capabilities of deep prediction models, providing improved accuracy in dynamic and evolving environments.
% as different samples may exhibit different types and extents of micro-drift, we introduce meta-learnable surrogate losses for each sample according to which the inferred latent embedding for the next period are adjusted to sample-specific ones to capture the micro-drift.

Moreover, for the problem of limited time series benchmark datasets for concept drift, we collect and open source three real-world electric load time series datasets. These datasets exhibit typical and diverse types of concept drift, making them ideal for evaluating and comparing different forecasting algorithms. 
% and diverse concept drift, creating realistic scenarios for evaluating the forecasting performance. 
To validate the effectiveness of LEAF, we conduct extensive experiments on the three electric load datasets as well as existing public benchmark datasets. 
Specifically, we apply LEAF to various types of deep prediction models, such as MLP, RNN, CNN, and Transformer-based models. Through evaluating LEAF's performance of different prediction models on datasets from various domains, we establish the universality and effectiveness of LEAF and highlight its robustness and applicability in addressing concept drift in online time series forecasting.
% The consistent superior performance of LEAF across different models and datasets highlights its robustness and applicability in addressing concept drift in online time series forecasting.


%%%To summarize, our contributions to this work are threefold:
%\vspace{-1mm}
%%%\begin{itemize}
   %\vspace{-2mm}
%%%    \item We propose the LEAF framework, a unified model-agnostic meta-learning framework that effectively addresses the challenges posed by concept drift in online time series forecasting. It learns to extrapolate and adjust the target prediction model in latent space and handle macro- and micro-drifts effectively.
    %\vspace{-1mm}
    
%%%    \item We open source three electric load time series datasets collected from real-world scenarios. These datasets exhibit diverse and typical concept drifts and are ideal benchmark datasets for the study of concept drift. We believe that real and challenging datasets can advance and promote the research of concept drift in time series. 
    %\vspace{-1mm}
    
%    , and introduce and analyze their characteristics and patterns of concept drift, providing realistic and challenging scenarios for evaluating forecasting models.
    
%%%    \item We conduct extensive experiments on multiple public and real-world time series benchmark datasets, demonstrating the superior performance of LEAF compared to existing approaches in various dynamic and evolving environments.
    
%%%\end{itemize}



==> 1-introduction_v2.tex <==
\section{Introduction}

%%%\emph{Paragraph 1. What is electric load forecasting and why it is important}

%%{\color{red} The organization of Paragraph 1.
%%\begin{itemize}
%%    \item What is electric load forecasting?
%%    \item Brief importance of electric load forecasting
%%    \item Introduction to MRELF, with an example in Fig. 1.
%%\end{itemize}
%%}

Electric load forecasting~\cite{ELF:2017:survey} predicts the future electricity demand based on historical data and other external factors such as weather forecast, economic factors, and other variables. 
It is crucial to balance supply and demand of power, reduce costs, and integrate renewable energy.
The traditional load forecasting generally performs at the aggregated level due to limited data. 
%%%lacks reliable prediction at lower gradu
%%%data quality issues and limited model capacities, granular predictions were unreliable. 
However, the rise of smart grids, smart meters, and multi-energy systems has provided access to more detailed and high-quality load data. In this paper, we focus on the Multi-region Electric Load Forecasting (MRELF) problem~\cite{Wu:MRELF:2022,Fan:MREFL:2010}.
%%Advances in deep learning now capture complex patterns at finer scales, facilitating the Multi-region Electric Load Forecasting (MRELF) problem~\cite{Wu:MRELF:2022,Fan:MREFL:2010}. 
As illustrated in Figure \ref{Fig_multi_region}, MRELF generates accurate short-term load predictions for multiple sub-regions within a large region.
Unlike the traditional single-region electric load forecasting, it considers the similarity and differences of difference regions to make the load prediction.

%%%which is crucial for maintaining the power grid’s supply-demand balance.


% % 第一段可以缩减。

% Electric load forecasting involves predicting future electricity demand, allowing utility companies, grid operators, and energy planners to make informed decisions about energy production, distribution, and infrastructure development. An accurate electric load forecast ensures a reliable balance between electricity supply and demand, preventing overloads and blackouts while optimizing resource allocation and minimizing operational costs. As the demand for electrical energy continues to rise, driven by technological advancements and increasing population growth, the need for accurate and reliable predictions of electricity consumption becomes ever more essential. 


% % 第一二段可以缩减后和在一起，重点是第二段
% {\color{red}Traditionally, load forecasting was conducted at an aggregated level due to significant challenges including data quality issues, lack of access to key influencing factors, and limited model capacities at more granular levels, which rendered lower-level forecasting less reliable. However, the advent of smart grids and smart meters, along with the integration of multi-energy systems, has provided utilities with access to more granular and higher-quality load data. Concurrently, advancements in deep learning models have enabled the capture of complex patterns at lower levels with remarkable precision. These developments facilitate more accurate predictions that take into account local variations, thereby enhancing resource allocation and localized risk management. This shift towards lower-level load forecasting exemplifies the Multiple Electric Load Forecasting (MRELF) problem, which aims to generate accurate load forecasts for multiple regions simultaneously.}

% {
% \color{blue} Electric load forecasting is crucial for utility companies to predict future electricity demand, ensuring a reliable balance between supply and demand, optimizing resource allocation, and minimizing operational costs. Traditionally, forecasting was performed at an aggregated level due to challenges like data quality issues, limited access to key factors, and constrained model capacities, making granular predictions unreliable. 

% However, the rise of smart grids and smart meters, coupled with the integration of multi-energy systems, has provided access to more detailed and higher-quality load data. Concurrent advancements in deep learning models have enabled the precise capture of complex patterns at finer levels, enhancing prediction accuracy. These developments support the Multi-region Electric Load Forecasting (MRELF) problem, which aims to generate accurate load predictions for multiple regions simultaneously, as shown in Figure \ref{Fig_multi_region}. As electrical energy demand grows with technological advancements and population increases, addressing the MRELF problem becomes essential for efficient and reliable energy management.
% }
% Multiple Electric Load Forecasting (MRELF) problem要不要改成多区域电力系统负荷预测Multi regional electric load forecasting 


% 这里可以添加一副图，展示负荷大区域与小区域的关系

\begin{figure}[!t]
  \centering
  \includegraphics[width=1\linewidth]{figures/multi-regional.pdf}\vspace{-3mm}
  \caption{Multi-region electric load forecasting. The main problem addressed in this paper is the short-term electric load forecasting problem for multiple sub regions (such as multiple cities) within a large region (such as the provincial level in the figure), which is of great significance for the supply-demand balance of the power grid.}
    \label{Fig_multi_region}
\end{figure}



%%\emph{Paragraph 2. Why accurate electric load forecasting is challenging?}

% 与一般的时序预测问题不同，一般的时序预测问题是只用过去的历史值对未来进行预测；但电力系统负荷预测涉及到协变量的参与，这些协变量对负荷的影响非常大。进行精准的电力系统负荷预测是非常有挑战的。1.对负荷的影响因子特别多，但是我们只能有有限的观测。2. 这些因子对负荷的影响在不同地区、不同时间的影响不一样。这在时间序列预测问题上称之为分布偏移问题。例如，温度同样上升一度，在7月1日，在东部沿海某省，靠近沿海的地市A负荷上升200w，而位于该省西部地区（完全内陆地市）温度同样上升了一度，负荷却上升了500w.对于该省的省会城市，春天温度变化一度和夏天温度变化一度，其负荷变化模式也展现出完全不同的特点。这些地区、时间的差异（偏移）在电力系统中是非常广泛存在的。3. 电力负荷的受到特殊的不确定因素。例如，环保限产。这些政策的颁布与实施通常是临时的，突然的，无法提前预知。4. 电力数据的质量问题。为了保证预测的及时性，预测所使用的历史负荷实时性较高。这些负荷数据采集自消费者端的传统或智能电表，这些设备容易出现传感器故障、传输问题、基础设施兼容性问题，进而导致数据噪声和缺失，这进一步限制了可利用的数据量。5. 在双碳目标的驱动下，新型电力系统的负荷结构更加多元化（例如分布式储能和电动汽车的大量接入），用户用电行为更加复杂，在环境、社会、经济等方面形成多维度的耦合关系，现有负荷模型难以精确描述用电负荷特性和分布规律。

% 但有趣的是，在对东部某省的电网调度相关数据进行详细的分析后，我们发现不同地市之间的负荷与协变量之间的关系存在共同性和特异性。具体来说，1. 不同地市之间影响因子与负荷之间的映射关系虽然存在差异，但是也有相似之处。这意味着在其他地市学习到的映射信息可以融合到目标地市的负荷预测中。2. 电力负荷与气象因素密切相关，但一个区域的气象因素只用有限个坐标点的气象是很难表达完全的，存在一些信息缺失。但由于区域之间的某些协变量实质上是紧密关联的（例如，相邻地市之间的气候相关程度高），所以设计合适的信息融合与迁移策略非常重要。这些策略可以动态自适应选择相似区域的信息来丰富目标区域的协变量特征。3. 待预测日的协变量在不同条件下（例如不同季节/气象）应该自动重点参照类似条件下的历史数据进行预测，这要求不同地市、不同时间的预测模型具备一定的特异性。

% {\color{blue}{Unlike conventional time series forecasting problems, electricity load forecasting relies not only on historical load data but also on a multitude of significant covariates. This dual dependency introduces substantial challenges in achieving accurate load predictions. Specifically, the primary difficulties are outlined as follows: 

% (i) Numerous Influencing Factors with Limited Observations: Electric load is affected by various factors such as temperature, humidity, economic activities, and holiday effects. However, in practice, the number of observable covariates is often restricted, making it difficult to comprehensively capture all influencing factors.

% (ii) Heterogeneity in Factor influence Across Regions and Time. The impact of covariates on load exhibits significant variations across different regions and time periods. For instance, an increase in temperature by 1°C on July 1st in a coastal city of an eastern province may result in a load increase of 200 MW, whereas the same temperature rise in an entirely inland city within the same province could lead to a 500 MW increase. Additionally, in a specific metropolitan area, a 1°C temperature change in spring may affect the load differently compared to the same change in summer. This regional and temporal heterogeneity, referred to as distributional shift, is pervasive in load forecasting and exacerbates the difficulty of achieving precise predictions.

% (iii) Impact of Special Uncertainty Factors: Electricity load is significantly influenced by unexpected and transient factors such as policy changes, for example, environmental production restrictions. The enactment and implementation of such policies are typically temporary and abrupt, making them difficult to anticipate in advance and thereby increasing the uncertainty in load forecasting.

% (iv) Data Quality Issues: To ensure real-time forecasting, historical load data utilized are often highly time-sensitive. These data are sourced from traditional or smart meters at the consumer end, which are susceptible to sensor malfunctions, data transmission problems, and infrastructure compatibility issues. Consequently, the data may contain noise and missing values, limiting the effectiveness and completeness of the available dataset.

% (v) Diversification of Load Structure and Complexity of Electricity Consumption Behavior: Driven by dual-carbon targets, the load structure in new electricity systems has become more diversified, with widespread integration of distributed energy storage and electric vehicles. This diversification leads to more complex user electricity consumption behaviors, creating multidimensional coupling relationships across environmental, social, and economic dimensions. Existing load models struggle to accurately describe the characteristics and distribution patterns of electricity load under these conditions, further complicating load forecasting efforts.
% }}

In this paper, we focus on the MRELF problem from a deep learning perspective. This problem not only inherits the complexities of traditional electric load forecasting but also places additional emphasis on flexibility and generality. {\color{blue} Specifically, traditional electricity load forecasting is inherently more complex than general time series prediction due to its dependence on a multitude of significant covariates alongside historical load data, thereby posing substantial challenges for achieving accurate predictions. Key difficulties include the wide range of factors that influence temperatures, humidity, levels of economic activity and holiday effects, which are often only partially observable, making it difficult to capture all relevant variables in a comprehensive way. Furthermore, the impact of these factors exhibits considerable regional and temporal heterogeneity, resulting in distributional shifts that complicate the precision of the prediction. The forecasting process is further impeded by unexpected uncertainty factors, such as abrupt policy changes (e.g., environmental production restrictions), data quality issues arising from sensor malfunctions and transmission problems in smart meters, and the diversification of load structures driven by dual-carbon objectives. } These issues  lead to more complex load behaviors and multidimensional couplings across environmental, social, and economic dimensions, result in a limited and fragmented training dataset characterized by noise and missing values, challenging existing deep learning models to accurately capture load characteristics and distribution patterns alone. 

% 这里regional variation、contextual variation, temporal variation分为三个点，分段描述，每段的定义/例子。加一个图，展示这三个点对于负荷预测的影响。

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/motivaton_plot.pdf}
    \caption{The motivation of regional, contextual, temporal variations.}
    \label{fig:motivation_plot}
\end{figure}

After conducting a comprehensive analysis of power grid data from various regions in a province in eastern China, we observed intriguing patterns in the relationships between load and covariates that revealing both commonalities and specificities among different regions, as shown in Figure \ref{fig:motivation_plot}. A significant finding is the pronounced similarity in electric load patterns across these regions. This similarity arises because electric load is a direct reflection of human activities, influenced by universal factors such as electricity pricing, daily routines, and weather conditions. Consequently, these shared influences contribute to the consistent emergence of peak load periods, particularly at night and noon, which are observed universally. Nevertheless, despite the similarities, the extent to which these factors impact the electric load varies significantly from three perspectives:
\begin{itemize}
    \item \textbf{Regional Variation}. This variation is largely attributable to regional differences in industrial structure and load composition. For instance, industrial hubs exhibit an increased sensitivity to electricity pricing, often adjusting production schedules in response to cost variations. In contrast, residential areas are more heavily influenced by climatic changes.
    \item \textbf{Contextual Variation}. The impact of influencing factors on electric load is highly dependent on the specific values of other covariates, referred to as the context. Certain covariates may exert more influence in particular situations. For instance, the impact of covariates such as temperature on electric load during a hot, rainy weekday in summer can differ significantly from their impact on a mild, windy holiday.
    \item \textbf{Temporal Variation}.  The influence of factors on electric load varies significantly over time throughout the day. For example, covariates such as temperature may have a lesser impact at dawn compared to their impact at noon on the same day.
\end{itemize}

 Ignoring the presence of region, context and temporal variations can lead to the gradient conflict problem \citep{chen2020just, liu2021conflict} in models, as samples from different areas and contexts may require distinct emphasis on various covariates, resulting in suboptimal performance and slower convergence rates. These insights highlight the necessity for more advanced models capable of leveraging information from multiple regions to extract both region-generic and region-specific features, thereby enhancing precision across regions in the presence of contextual and temporal variations.

To achieve the above objective, the existing literature predominantly offers two main categories of methods. The first category of methods utilizes Graph Neural Networks to capture the dependency across different regions \citep{mansoor2024graph, chen2023research}. However, these methods often demand a significant amount of prior knowledge to construct the graphs effectively. They also face challenges related to data quality and distribution shifts, which are common in MRELF, leading to overfitting and diminished model performance. Alternatively, by considering each region as a distinct task, the problem of MRELF can be naturally formulated within the framework of Multi-Task Learning (MTL). MTL provides various techniques to facilitate the learning of both region-generic and region-specific components \citep{fiot2016electricity, jiang2021hybrid, jiang2021hybrid, liu2023boosted}. Nonetheless, these methods often require extensive manual customization, which compromises their general applicability, increases computational costs, and may result in gradient conflicts, hindering forecasting accuracy due to overlooking regional, contextual, and temporal variations. 

Recently, the development of Mixture of Experts (MoE) methods \citep{chen2023mod, ye2023taskexpert, yang2024multi} within the MTL framework has shown significant potential in addressing gradient conflict issues among tasks. Despite their promises, the applicability of MoE methods to MRELF remains largely unexplored, as existing research primarily focuses on applications in the vision or language domain with abundant data and transformer-based architectures.

To bridge these gaps, we introduce a new model, TriForecaster, which innovatively addresses the MRELF problem by using mixtures of MoE within the MTL framework. TriForecaster enables flexible cooperation and specialization of experts across regional, contextual and temporal dimensions which further enhances the model's ability to leverage region-general information while simultaneously adapting to distinct regional, contextual, and temporal characteristics. Firstly, the model extracts and integrates both region-specific and region-generic information using stacks of RegionMixer layers. Within each layer, a shared general model captures region-generic features that are relevant across various regions, while distinct region-specific expert models focus on unique, localized attributes. The integration of these diverse features is achieved using a parameter-efficient stochastic fusion module \citep{han2024softs}, which intelligently combines information by assessing similarities between expert models. This method eliminates the need for region-specific gating networks and load balance auxiliary loss within each layer while leveraging both region-specific and aggregated information from all experts to enhance local adaptations\citep{han2024softs}. Subsequently, the integrated information within each layer undergoes processing through a series of Context-Time Specializer (CTSpecializer) layers to accommodate contextual and temporal variations. Specifically, a context-mixing MoE module is applied to the feature dimension, mixed by the stochastic fusion, and is followed by time-mixing MoE module applied to the temporal dimension, also processed by a stochastic fusion. This sequential processing ensures comprehensive accommodation of contextual and temporal variations. Experimentally, TriForecaster demonstrates superior performance compared to state-of-the-art models on four real-world MRELF datasets collected from diverse global locations, with varying levels of granularity from city to bus level. These results underscore TriForecaster's exceptional performance, flexibility, and general applicability across different contexts and scales. 

{\color{red}add other advantages of our framework, 
1. more samples, 2. }

We outline our contributions as follows:
\begin{enumerate}
    \item Motivated by commonalities and specificities among different regions in a province in eastern China, we propose a novel approach to tackle the Multi-Regional Electricity Load Forecasting (MRELF) problem. Our approach emphasizes the importance of effectively leveraging region-generic information while also attentively addressing the variations across regional, contextual, and temporal dimensions. To the best of our knowledge, this approach is the first to tackle the MRELF challenge from this specific perspective.
    \item We introduce TriForecaster, a framework featuring the RegionMixer layer and the CTSpecializer layer, designed to enable flexible cooperation and specialization of experts across regional, contextual, and temporal dimensions, facilitated by a parameter-efficient stochastic fusion mechanism.
    \item Experimental results on four real-world MRELF datasets from diverse global locations, with varying levels of granularity from city to bus level, demonstrate the state-of-the-art performance, flexibility, and generality of TriForecaster.
    \item TriForecaster has been integrated into our eForecaster platform \citep{eForecaster2023} and deployed in a province in eastern China. It provides city-level short-term load forecasting for 17 cities, covering a population of over 110 million people and daily electricity usage exceeding 100 gigawatt-hours.
\end{enumerate}

{\color{red} Discuss the contributions. 1 (identifying the challenges) may not be a strong contribution. 2 can be further splitted into 2. }

% the relationships between load and covariates across different cities exhibit both commonality and specificity. Although the mapping between influencing factors and load varies among cities, underlying similarities suggest that information learned from one city can be integrated into the load forecasting of another. Moreover, while electricity load is closely related to meteorological factors, accurately representing regional meteorological conditions with a limited number of coordinate points is challenging, resulting in information loss. However, inherent correlations among covariates across regions, such as high climate similarity among neighboring cities, underscore the importance of effective information fusion and transfer strategies. These strategies should dynamically and adaptively incorporate data from similar regions to enhance the covariate features of the target region. Additionally, forecasting models must prioritize historical data from analogous conditions (e.g., similar seasons or weather patterns) to improve prediction accuracy, necessitating a degree of specificity tailored to different cities and temporal contexts. These insights highlight the need for advanced, robust forecasting models that can leverage shared information while accommodating regional and temporal specificities to enhance the precision of electricity load predictions.}



% Electric load forecasting is inherently more complex than traditional time series forecasting, as it heavily depends on various covariates like weather conditions, policy changes, electricity pricing structures, as well as their interactions alongside intricate temporal variations. For example, temperature influences electricity load more significantly in the summer  compared to the spring because of increased cooling demands, with its effects amplified during consecutive hot days due to accumulated heat stress. These complexities are exacerbated by data quality and availability issues, making it even more challenging to discern the underlying relationships. Specifically, electric load is significantly affected by external events and extreme weather conditions, such as holidays, heatwaves, and heavy snowfalls. However, the infrequent occurrence of these events in historical data poses substantial challenges for forecasting. In addition, electricity data is typically collected from smart or traditional meters located at consumer sites, a process prone to difficulties such as measurement errors, sensor failures, data transmission issues, and infrastructure upgrades. These challenges result in a limited and fragmented training dataset characterized by noise and missing values. Developing forecasting models in this context often leads to overfitting, making it difficult to accurately uncover the true relationships between loads and their covariates. 

% {\color{red}Here focus on the tabular data problem, how to incorporate covariates in forecasting.}
% Multi-Task Learning (MTL) focuses on optimizing multiple tasks simultaneously. Its ability of learning shared relationship, often referred to as \textbf{cooperation}, while maintaining discriminative task-specific information, known as \textbf{specialization}, makes it an ideal approach for addressing the aforementioned challenges. This paradigm is particularly beneficial in the context of electricity data, as it allows for the exploitation of information from multiple regions, thereby enhancing forecasting accuracy and robustness. Nonetheless, identifying optimal strategies for cooperation and specialization—such as determining where, how, and what information to share—remains a challenge in electricity load forecasting. Previous works ~\citep{9462500} uses MTL to ... 

% 1) hand-crafted architecture
% 2) complexcity
% 3) focus more on the cooperation

% In this paper, we seek the answer to the question: \textit{How can we effectively cooperate and specialize information from multiple regions to uncover the dependency of electrical load on various covariates along with their interactions amid complex temporal variations?} We explore the intricacies of cooperation and specialization and their interplay with covariates under temporal variations in multiple regions through two lenses linked to the characteristics of electric load data. Firstly, we note that while different regions may share some common features, they also possess unique demand drivers. For example, industrial hubs are more sensitive to electricity pricing to plan production schedules, whereas residential areas are more influenced by climate changes. These variations result in distinct dependency patterns on covariates, even among geographically proximate areas. This observation highlights the necessity of extracting both region-generic and region-specific representations that effectively utilizes shared knowledge, while capturing local covariate dependencies and consumption patterns. On the other hand, ...
%  For example, when forecasting the daily electric load 
% % perform joint learning over multiple regions, they mainly focus on how to perform coorperation where they incorporate same encoder to extract shared knowledge with task-specific decoders. However, these approaches ignores the significant regional differences where nearby regions have different demand drivers which leads to the conflict gradient problem.

% % The regional differences make the problem even more challenging where nearby regions have different demand drivers such as industrial hubs or residential areas which leads to different dependency patterns on covariates, necessitating regional-specific forecasting models that account for local covariates dependencies and consumption patterns.

% % Co-variates dependency (Integration of Renewable Energy, Weather Dependency, )
% % Data Quality and Availability ( Accurate forecasting relies heavily on historical data, but inconsistencies, gaps, or inaccuracies in data collection can hamper forecast precision. Ensuring data quality and integrating various data sources is a complex task. Technological and Behavioral Changes)
% % Short-term Events and Anomalies
% % Regional difference


% \emph{Paragraph 3. Multi-task learning seems a good direction but very few or shadow research has been permformed in this area. List some simple related work.}



% \emph{Paragraph 4 (or 4 and 5). Address our contributions in detail, including: 1) our technical novelty and advancement; 2) our improvements in electric load forecasting; 3) deployment.}

==> 4-methodology_v2.tex <==
% \vspace{-3mm}
\section{Methodologies}
% \vspace{-3mm}

\subsection{Problem Formulation}
% \vspace{-2mm}
The problem of electric load forecasting is a specific aspect of the broader multivariate time series forecasting problem. In this section, we will sequentially introduce the concepts of multivariate time series forecasting, electric load forecasting, and multi-region electric load forecasting.


\textbf{Multivariate Time Series Forecasting.}\hspace{0.5mm} Given history observations $\mathbf{S} \in \mathbb{R}^{L \times C}$, where $L$ is the length of lookback window and $C$ is the number of channels. The goal of multivariate time series forecasting is to learn a predictive model $F_{\boldsymbol{\theta}}$ to predict future values $\mathbf{Y} \in \mathbb{R}^{H \times C}$ where $H > 0$ is the forecast horizon. 

\textbf{Electic Load forecasting.}\hspace{0.5mm} Electricity load forecasting extends beyond historical data, incorporating future covariates such as weather forecasts and date features that influence electricity consumption. Given historical observations $\mathbf{S} \in \mathbb{R}^{L \times C}$ and future covariates $\mathbf{Z} \in \mathbb{R}^{H \times C_z}$, denoted collectively as $\mathbf{X} = (\mathbf{s}, \mathbf{z})$, the objective is to learn a predictive model $F_{\boldsymbol{\theta}}$. This model aims to forecast future electricity load demands $\mathbf{y} \in \mathbb{R}^{H \times 1}$, formalized as: $\mathbf{X} \xrightarrow[]{{F}(\cdot;{\boldsymbol{\theta}})}  \mathbf{y}$.

\textbf{Multi-region Electric Load Forecasting via MTL.}\hspace{0.5mm} 
Assume there are $T$ different regions, MELF seeks to simultaneously predict future electric load for these regions. This is conceptualized as a MTL problem, where each region is defined as a distinct task $\{\mathcal{T}_1, \ldots, \mathcal{T}_T\}$. For each region $t$, there is an associated dataset $\mathcal{D}_t = \{(\mathbf{X}^t_i, \mathbf{y}^t_i)\}_{i=1}^{N_t}$, where $\mathbf{X}^t_i$ represents the composite input features, including historical observations and future covariates, and $\mathbf{y}^t_i$ denotes the target load demand. The objective is to learn a predictive model $F(\cdot)$ using a shared set of parameters $\boldsymbol{\theta}_s$ applicable across all regions, as well as region-specific parameters $\{\boldsymbol{\theta}_t\}_{t=1}^{T}$ for each individual task. The learning problem can be formulated as an optimization problem, aiming to minimize the cumulative loss across all regions:

\[
\min_{\boldsymbol{\theta}_s, \{\boldsymbol{\theta}_t\}_{t=1}^{T}} \sum_{t=1}^{T} \frac{1}{N_t}\sum_{i=1}^{N_t} \mathcal{L}(F(\mathbf{X}^t_i; \boldsymbol{\theta}_s, \boldsymbol{\theta}_t), \mathbf{y}^t_i)
\]

% \textcolor{blue}{add some discussion? mainly focus on the challenges of solving above problem. commented by linxiao}



% predictive model $F_{\boldsymbol{\theta}_}$ $\mathbf{X} = \{\}$ ates $\boldsymbol{z} \in \mathbb{R}^{H \times C_z}$, denoted collectively as $\mathbf{x} = (\boldsymbol{s}, \boldsymbol{z})$, the objective is to learn a predictive model $F_{\boldsymbol{\theta}}$. This model aims to forecast future electricity load demands $\mathbf{y} \in \mathbb{R}^{H \times 1}$, formalized as: $\mathbf{x} \xrightarrow[]{{F}(\cdot;{\boldsymbol{\theta}})}  \mathbf{y}$.


% \textbf{Multivariate time series forecasting.}\hspace{0.5mm} A multivariate time series is an ordered sequence of observations denoted $\mathcal{A} = ( \boldsymbol{a}_1, \boldsymbol{a}_2, \cdots,\\ \boldsymbol{a}_T ) \in \mathbb{R}^{T \times c}$, where $T$ is the total number of time steps, $\boldsymbol{a}_i\in\mathbb{R }^c$, and $c$ is the multivariate dimension. Multivariate time series forecasting aims to learn a predictive model ${F}_{\boldsymbol{\theta}}$ to predict the next $P$ steps at time $t$ given a look-back window of length $L$ as $\boldsymbol{a}_{t-L+1:t}  \xrightarrow[]{{F}(\cdot;{\boldsymbol{\theta}})}  \boldsymbol{a}_{t+1:t+P}$, where $\boldsymbol{\theta}$ is the model parameter. 

%For simplicity, in the remainder of the paper, we denote the input  $\boldsymbol{z}_{t-I+1:t}$ and the output $\boldsymbol{z}_{t+1:t+O}$ as $\mathbf{x}$ and $\mathbf{y}$ and a set of input and output as $\mathbf{X}$ and $\mathbf{Y}$, respectively.

% In this section, we first introduce traditional time series forecasting setting, then we extend this setting to online time series forecasting. For a multivariate time series of $T$ observations and $C$ channels: $\mathbf{Y}_{1:T} = (\mathbf{y}_1, \mathbf{y}_2, ...,\mathbf{y}_T) \in \mathbb{R}^{T \times C}$, where each element $\mathbf{y}_t \in \mathbb{R}^C$ is a $C$-dimensional vector, the $t$th sample from a subsequence $\mathbf{Y}_{S:E}$ of the time series is defined as a pair $(\mathcal{X}^{(S)}_t, \mathcal{Y}^{(S)}_t)$, where $\mathcal{X}^{(S)}_t$ is a lookback window of length $L$ starts from time $S$: $\mathcal{X}^{(S)}_t := \mathbf{Y}_{S + t - 1:S + t + L - 1} = (\mathbf{y}_{S + t - 1},...,\mathbf{y}_{S + t + L - 1}) \in \mathbb{R}^{L \times C}$ and $\mathcal{Y}_t$ is a forecast horizon of length $H$ starts from time $S$: $\mathcal{Y}_t := \mathbf{Y}_{S + t + L: S + t + L + H -1} = (\mathbf{y}_{S + t + L},...,\mathbf{y}_{S + t + L + H -1}) \in \mathbb{R}^{H \times C}$. Denote the dataset constructed from $\mathbf{Y}_{S:E}$ by $\mathcal{D}_{S, E} = \{(\mathcal{X}^{(S)}_t, \mathcal{Y}^{(S)}_t)\}^{|\mathcal{D}_{S, E}|}_{t=1}$, where $|D_{S, E}| = E - S - H - L + 2$ is the size of the dataset. The goal is to fit a forecaster $f_{\theta} (\cdot): \mathbb{R}^{L \times C} \rightarrow \mathbb{R}^{H \times C}$ on $\mathcal{D}_{1,T}$ that minimizes some loss function $\mathcal{L}$.


% \textbf{Load forecasting.}\hspace{0.5mm} In the context of load forecasting, electricity load prediction is not only affected by historical load data, but also by other auxiliary factors such as meteorological factors, date factors and so on. For example, meteorological factors may include temperature, humidity, wind speed, precipitation, etc., and date factors can include holidays and days of the week. Unlike the general time-series forecasting problem, when doing load forecasting the future auxiliary variables are always available. That is, we can predict tomorrow's load based on information such as tomorrow's weather forecast and whether tomorrow is a workday. Therefore, we can organize the relevant data in the historical sequence: $\boldsymbol{s} \in \mathbb{R}^{L \times c}$, the future sequence: $\boldsymbol{u} \in \mathbb{R}^{P \times (c-1)}$ and the target sequence: $\boldsymbol{t} \in \mathbb{R}^{P \times 1}$, . Based on this, we can formulate the load forecasting problem as: $(\boldsymbol{s},  \boldsymbol{u}) \xrightarrow[]{{F}(\cdot;{\boldsymbol{\theta}})}  \boldsymbol{t}$. For simplicity, in the remainder of the paper, we denote the input  $(\boldsymbol{s},  \boldsymbol{u})$ and the output $\boldsymbol{t}$ as $\mathbf{x}$ and $\mathbf{y}$ and a set of input and output as $\mathbf{X}$ and $\mathbf{Y}$, respectively.
% Time series data often arrives in a streaming fashion with frequent concept drift. %Traditional approaches training a prediction model once and evaluating it separately are unsuitable. Instead, 
% An appropriate approach is to continuously update the model over a sequence of periods. At each online forecasting period $p$, the model accesses and learns from the most recent data available and makes predictions for the future. Subsequently, the ground truth is revealed, allowing for updating the model once again. 
% In online forecasting settings, the model is iteratively updated at regular periods, referred as online forecasting period, and then evaluated on the next period of incoming data. 
% Moreover, online forecasting often does not start from scratch, and we warm up the model based on historical data.
% Figure \ref{fig:online_time_series_forecasting} provides a visual representation of the procedure involved in online time series forecasting.

 
% \textbf{Multi-region load forecasting.}\hspace{0.5mm} Users in different regions have different patterns of power consumption, so regional relationships are also considered as a load-influencing factor. When considering load forecasting across multiple regions, things may be a little different. Assuming there are $N$ regions in consideration, the multi-region load forecasting seeks to learn a set of prediction models $F(\cdot;\boldsymbol{\theta}_i), i \in \{1,\cdots,N\}$ to predict next $P$ steps load values given past historical information and future auxiliary variables:
% $$
% \mathbf{x}_i \xrightarrow[]{F(\cdot;\boldsymbol{\theta}_i)} \mathbf{y}_i, \qquad i \in \{1,\cdots,N\}
% $$
% where $\mathbf{x}_i = (\boldsymbol{s}_i, \boldsymbol{u}_i)$ represents the input variables of the $i^{\text{th}}$ region, and $\mathbf{y}_i = \boldsymbol{t}_i$ represents the target load sequence of the $i^{\text{th}}$ region. 

% As mentioned above, when we design these $N$ models, we need to explicitly model their cooperation and specialization to make prediction more accurately. To achieve this goal, we propose a novel model named \textcolor{red}{TriForecaster}, which consists of a two-stage mixture of experts and a novel fusion mechanism that can fetch and fuse information from different branches. 

% Note that simply fitting a prediction model to the most recent observed data is insufficient due to concept drift, and the model needs to effectively generalize to future data. This requires a meta-learning approach. Meta-learning, also known as learning to learn, is a machine learning approach where a model learns how to learn from experience or previous tasks, enabling it to quickly adapt and generalize to new tasks. In the context of online time series forecasting, our objective is to learn how to adapt to future data. 
% % To address this challenge, we propose a meta-learner called LEAF. 
% Our meta-learning based LEAF algorithm is trained over a sequence of online forecasting periods, referred as the meta-training phase, and evaluated over another sequence of periods called the meta-test phase. The procedure is depicted in Figure \ref{fig:online_time_series_forecasting}. 

% \textbf{Macro- and micro-drifts.}\hspace{0.5mm} 
% Macro-drift refers to drifts that are stable and persist over relatively long duration. Here, macro-drift can be measured using the symmetric KL divergence between two adjacent periods of data. The magnitude of the macro-drift of period $p$ can be computed as \footnote{Here we only consider the univariate situation. As for multivariate times series, we can sum the KL divergence of each dimension.}

% \begin{equation}
% \begin{aligned}
% \mathrm{KL}_{\text {avg }}\left(P_{p}, P_{p-1}\right) & =\frac{1}{2}\left\{\mathrm{KL}\left(P_{p} \| P_{p-1}\right)+\mathrm{KL}\left(P_{p-1} \| P_{p}\right)\right\} \\
% & =\frac{1}{2} \int\left(P_{p}(z)-P_{p-1}(z)\right) \log \frac{P_{1}(z)}{P_{0}(z)} dx.
% \end{aligned}
% \end{equation}

% Assume that the data follow Gaussian distribution, i.e., $P_{p}(z) \sim \mathcal{N}(\mu_{p},\sigma_{p}^{2})$, we have 


% \begin{equation}
% \small
% \begin{aligned}
% \mathrm{KL}_{\text{avg}}\left(P_{p}, P_{p-1}\right)=\frac{1}{2}\left(\frac{1}{2 \sigma_{p}^{2}}+\frac{1}{2 \sigma_{p-1}^{2}}\right)\left[\left(\mu_{p}-\mu_{p-1}\right)^{2}+\left(\sigma_{p}^{2}-\sigma_{p-1}^{2}\right)^{2}\right]
% \end{aligned}
% \end{equation}

% In contrast, micro-drift characterizes abrupt, transient changes, which can be considered as outlier samples. Here, micro-drift can be measured as Euclidean distance between a sample and the averaged sample in the same period. The magnitude of micro-drift of sample $[x;y]$ can be computed as

% \begin{equation}
% \begin{aligned}
% \mathrm{EUC}\left([x;y], [\overline{x};\overline{y}] \right) = \left([x;y] -  [\overline{x};\overline{y}]\right)^2,
% \end{aligned}
% \end{equation}

% where $[\dot;\dot]$ denotes the concatenation operation, and $\overline{x}$ and $\overline{y}$ are the averaged ${x}$ and ${y}$ in the period, respectively.

% \begin{figure}[!t]
%  % \vspace{-10mm}
%     \centering
%     \includegraphics[width=0.48\textwidth]{figures/online_forecast.pdf}
%     % \vspace{-5mm}
%     \caption{Illustration of online time series forecasting via LEAF. LEAF is a meta-model that guides the optimization of the prediction model $f_{\boldsymbol{\theta}}$.}
%     \label{fig:online_time_series_forecasting}
%     % \vspace{-5mm}
% \end{figure}

% By harnessing the meta-learning capabilities of LEAF, we empower the prediction model to adeptly adapt and make accurate forecasts in the presence of concept drift.

% Note that fitting a prediction model up-to-date accodring to the recently observed data is not enough, as the model needs to be applied to future data which might come from a different environment and exhibit different characteristics due to the frequent concept drift. As a result, a prediction model should rather adapt to future data which calls for meta-leaning. Meta-leaning [meta-learning], also known as learning to learn, is a machine learning approach where a model learns how to learn from experience or previous tasks, enabling it to quickly adapt and generalize to new tasks. Our problem here is learning to adapt the future. To solve this problem, we introduce a meta-leaner (LEAF), which is trained over a sequence of online forecasting periods and evaluated over another sequence, which are called meta-training and meta-test phase, respectively.

% In online scenarios, future data comes over time as streams $(\mathbf{y}_1, \mathbf{y}_2, ..., \mathbf{y}_T, ....)$. The forecaster is first trained on warm up time series $\mathbf{Y}_{1:T}$ with warm up length $T$, denote $\mathcal{D}^{warm}$ as the warm up dataset, then the forecaster is deployed online at $T+1$. For each online step $k \geq 1$,  the forecaster is updated on dataset $\mathcal{D}_k := \mathcal{D}_{T+(k-1)s + 1, T + ks}$ constructed from $\mathbf{Y}_{T+(k-1)s+1:T + ks}$ where $s$ is the online step size, then make predictions for every lookback windows in the future dataset $\mathcal{D}_{k+1}$. Lastly, the loss $\mathcal{L}^{\mathcal{D}_{k+1}}$ is calculated after receiving the targets. This procedure provides a natural choice for task splitting for meta-learning. Specifically, we define a sequence of tasks $\mathcal{T} = (\mathcal{T}_1, \mathcal{T}_2, ....)$. For each online step $k$, the task $\mathcal{T}_k$ consists $(\mathcal{D}^S_k, \mathcal{D}^Q_k)$, where $\mathcal{D}^S_k := \mathcal{D}_k$ is the support set and  $\mathcal{D}^Q_k := \mathcal{D}_{k+1}$ is the query set. Thus, at each online step $k$, from a bi-level optimization view, we first digest dataset $\mathcal{D}_k$ to obtain the task-specific parameters; next, we make predictions for dataset $\mathcal{D}_{k+1}$; then, we obtain the targets for $\mathcal{D}_{k+1}$ and calculate the loss $\mathcal{L}^{\mathcal{D}_{k+1}}$; finally, we update the meta-learner base on the loss. Notice that, within each task, concept drift could occur between $\mathcal{D}^S$ and $\mathcal{D}^Q$, that is $P^S(\mathcal{X}, \mathcal{Y}) \neq P^Q(\mathcal{X}, \mathcal{Y})$. According to [], the concept drift can be split into conditional distribution shift $P^S(\mathcal{Y} | \mathcal{X}) \neq P^Q(\mathcal{Y} | \mathcal{X})$ and covariates shift $P^S(\mathcal{X}) \neq P^Q(\mathcal{X})$ which will be alleviated explicitly in  Meta-TS$^2$Net.


% \subsection{Test-time Adaptation}
% \vspace{-2mm}
\subsection{TriForecaster}
% \vspace{-2mm} 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/architecture_plot.pdf}
    \caption{The architecture of our proposed TriForecaster model.}
    \label{fig:model}
\end{figure*}
% \vspace{-2mm}
% \vspace{-2mm}
An overview of the proposed \textit{TriForecaster} framework is presented in Figure \ref{fig:model}. Our methodology introduces the RegionMixer module, which is devised to integrate region-specific and region-generic information comprehensively across all regions. This integrated information is subsequently processed by the CTSpecializer component, which is engineered to effectively capture both contextual and temporal variations. The final electric load forecasts are generated by employing a region-specific projection head on the latent embeddings, which are enriched with a synergistic blend of region-generic, region, contextual, and temporal-specific information.
% Firstly, the input sequences are fed into a \textcolor{red}{RegionMixer} block where samples from different regions are assigned to different experts. The information from other experts is then integrated through the proposed fusion mechanism. The output latent of the \textcolor{red}{RegionMixer} block is sent to the next \textcolor{red}{CTSpecializer} block, which consists of two modules, namely \textcolor{red}{TimeMoE} and \textcolor{red}{CovariateMoE}. This block is mainly used for encoding cooperation among all regions. We also add a contrastive loss to encourage each expert to focus on processing similar samples. Finally, the latent representation is used for generating the corresponding region predictions with a specialized prediction head. Details are provided in the following several sections.


% \vspace{-2mm}
\subsubsection{RegionMixer}
\label{section:regionmixer}
As shown in Figure \ref{fig:model}, the raw input $\mathbf{X}^{t}$ for region $t$ first goes through an embedding layer $\text{Embedding}(\cdot)$ that projects historical observations with length $L$ to future forecast horizon length $H$ and produce initial latent representation $\mathbf{X}^{t, 0} \in \mathbb{R}^{H \times d_r}$ where $d_r$ is the dimension of the latent space. The latent representation $\mathbf{X}^{t, 0}$ is subsequently processed through $N_r$ stacked RegionMixer layers, each augmented with residual connections \citep{he2016deep}. For a layer $l \in \{1,\cdots,N_r\}$ with the input $\mathbf{X}^{t, l-1} \in \mathbf{R}^{H \times d_r}$, the process is formulated as:
\begin{equation}
\begin{aligned}
\mathbf{X}^{t, l} = \text{RegionMixer}(\mathbf{X}^{t, l-1}) + \mathbf{X}^{t, l-1}.
\end{aligned}
\end{equation}
For each layer \( l \), the architecture incorporates \( T \) region-specific expert functions \( \{ f^{t,l}: \mathbb{R}^{H \times d_r} \mapsto \mathbb{R}^{H \times d_r} \}_{t=1}^T \) (where \( T \) denotes the total number of geographical regions), each specialized to encode localized spatiotemporal patterns unique to region \( t \). A shared expert function \( f^{0,l}: \mathbb{R}^{H \times d_r} \mapsto \mathbb{R}^{H \times d_r} \) concurrently models global dynamics common across all regions. Given an input instance \( \mathbf{X}^{t,l}_n \in \mathbb{R}^{H \times d_r} \) from region \( t \) (where \( n \) indexes samples within a batch), the corresponding regional and shared representations are computed as:  
\[
\mathbf{O}^{t,l}_n = f^{t,l}(\mathbf{X}^{t,l}_n), \quad \mathbf{O}^{0,l}_n = f^{0,l}(\mathbf{X}^{t,l}_n),
\]  
both residing in \( \mathbb{R}^{H \times d_r} \). Let \( o^{t,l}_{n,j,k} \in \mathbb{R} \) denote the activation at position \( (j,k) \) of \( \mathbf{O}^{t,l}_n \), and \( f^{t,l}_{j,k} \) represent the functional component generating this activation. It is important to note that \(f\) can be any time series forecasting model. In this study, we specifically employ the TSMixer \citep{chen2023tsmixer}. Layer indices \( l \) are omitted in subsequent equations where unambiguous.

% The general model, \(f^0\), captures global relationships between load and covariates that are consistent across all regions, whereas the models \(f^t\) are designed to encode region-specific relations. Note that the function \(f\) may represent any time series forecasting model; in this study, we utilize the TSMixer.}

% Concretely, we can denote the region-experts as $f^i, i \in \{1,\cdots,N\}$ and the general-expert as $f^0$ respectively. Here $N$ is the number of all regions in consideration. Each expert $f$ can be viewed as projecting the input variables into a common latent space for later processing. 
% For a sample $\mathbf{x}^i$ of the $i^{\text{th}}$ region, its specialized latent and shared latent can be denoted as $f^i(\mathbf{x}^i)$ and $f^0(\mathbf{x}^i)$, respectively. Here, $f^0$ can be viewed as the global relationship between load and covariates shared by all regions, and $f^i$ plays the role of encoding region-specific load-covariate relationships.
Effective regional cooperation necessitates integration of both global dependencies and localized pairwise interactions. While prior work \citep{chen2023mod, ye2023taskexpert, yang2024multi} employs task-specific gating networks with Top-K expert selection and auxiliary loss regularization to induce sparsity, such approaches incur prohibitive computational overhead and risk suboptimal expert specialization due to artificial workload balancing constraints.

\textbf{Pairwise interaction}. Drawing inspiration from STAR's channel interaction mechanism \citep{han2024softs}, we propose a parameter-efficient alternative through component-wise stochastic fusion. For region $t$, we construct a 3D probability tensor $\mathbf{P}^t \in \mathbb{R}^{T \times H \times d_r}$ quantifying pairwise expert affinities for each temporal position $j \in \{1,\cdots, H\}$ and latent dimension $k \in \{1,\cdots,d_r\}$. Given a mini-batch of $N$ samples $\{\mathbf{X}^{t}_n\}_{n=1}^N$, the affinity between expert $t$ and expert $i \neq t$ at position $(j,k)$ is computed as:  
\begin{equation}  
d(f^{t}_{j,k}, f^{i}_{j,k}) = \sum_{n=1}^N \left| o^{t}_{n,j,k} - o^{i}_{n,j,k} \right|, 
\end{equation}  
yielding the categorical distribution:  
\begin{equation}  
\mathbf{P}^t_{:,j,k} = \text{Softmax}\left( -\left[ d(f^{t}_{j,k}, f^{i}_{j,k}) \right]_{i \in \{0,\ldots,T\}\setminus\{t\}} \right),
\end{equation}  
This procedure of calculating pairwise affinities eliminates region-specific gating networks by directly measuring component-wise expert similarity through batch statistics. 

\textbf{Stochastic fusion mechanism}. 
Let $\mathbf{O}_{\text{cat}} = \{\mathbf{O}^i\}_{i \in \{0,\ldots,T\}\setminus\{t\}}\in \mathbb{R}^{T \times H \times d_r}$ be the concatenated outputs of experts. The Fusion module:
\begin{equation}  
\mathbf{X}^t = \text{Fusion}(\{\mathbf{O}^t, \mathbf{O}^0\}, \mathbf{O}_{\text{cat}}, 
\mathbf{P}^t) \in \mathbb{R}^{H \times d_r},
\end{equation} 
synthesizes regional ($\mathbf{O}^t$), global ($\mathbf{O}^0$), and pairwise ($\mathbf{O}_{\text{pair}}$) information through:  
\begin{equation}  
\begin{aligned}  
\mathbf{O}_{\text{cat}} &= \text{FFN}_1\left( \mathbf{O}_{\text{cat}} \right) \in \mathbb{R}^{T \times H \times d_r} \\  
\mathbf{O}_{\text{pair}} &= \text{Stoch\_Pool}(\mathbf{O}_{\text{cat}}, \mathbf{P}^t)\\  
\mathbf{X}^t &= \text{FFN}_2\left( \text{Concat}(\mathbf{O}^t, \mathbf{O}^0, \mathbf{O}_{\text{pair}}) \right) \in \mathbb{R}^{H \times d_r}  
\end{aligned}  
\end{equation}  
where $\text{FFN}_1: \mathbb{R}^{d_r} \to \mathbb{R}^{d_r}$ and $\text{FFN}_2: \mathbb{R}^{3d_r} \to \mathbb{R}^{d_r}$ are feed-forward networks, Concat operator concatenate the inputs on the latent dimension, and $\text{Stoch\_Pool}(\mathbf{O}_{\text{cat}}, \mathbf{P}^t) \in \mathbb{R}^{H \times d_r}$ implements a stochastic pooling mechanism defined as:
\begin{equation}
\begin{aligned}
(o_{\text{pair}})_{j, k} = (o_{\text{cat}})_{e, j, k} \quad \text{where} \; e \sim \text{Categorical}(\mathbf{P}^t_{:, j, k}).
\end{aligned}
\end{equation}

This module improves the expressiveness of RegionMixer by allowing each temporal position and latent dimension to select freely among experts. At the same time, by utilizing the stochastic pooling, it encourages the exploration over experts while removing the need for auxiliary loss.

% Next, the probability tensor is used in the Fusion module to random select which expert to attend, where the result parwise information $\mathbf{H}_{\text{pair}} \in \mathbb{R}^{H \times d_r}$ is later aggregated with region-specific information and global information. Let $\mathbf{H} = \{\mathbf{O}^i\}_{i \in \{0, \cdots, T\} \setminus \{t\}} \in \mathbb{R}^{T \times H \times d_r}$, the process of Fusion can be formulated as:
% \begin{equation}
% \begin{aligned}
% \mathbf{H} &=  \text{FFN\_1}(\mathbf{H}),\\
% \mathbf{H}_{\text{pair}}&= \text{Stoch\_Pool}(\mathbf{H}, \mathbf{P}^t),\\
% \mathbf{X}^t &= \text{FFN\_2}\left(\text{Concat}(\mathbf{O}^t, \mathbf{O}^0, \mathbf{H}_{\text{pair}})\right),
% \end{aligned}
% \end{equation}
% Where $\text{FFN\_1}: \mathbb{R}^{d_r} \mapsto \mathbb{R}^{d_r}$, $\text{FFN\_2}: \mathbb{R}^{3d_r} \mapsto \mathbb{R}^{d_r}$ are two linear layers, Concat operator concatenate the inputs on the latent dimension. 
% $\text{Stoch\_Pool}(\mathbf{H}, \mathbf{P}^t) \in \mathbb{R}^{H \times d_r}$ select from $\mathbf{H}$ according to a categorical distribution over experts based on $\mathbf{P}^t$ for each future forecast horizon $j$ and latent dimension $k$:
% \begin{equation}
% \begin{aligned}
% (h_{\text{pair}})_{j, k} = h_{e, j, k} \quad \text{where} \; e \sim \text{Categorical}(\mathbf{P}^t_{:, j, k}),
% \end{aligned}
% \end{equation}


% between regions by computing the similarities between $\{f^t\}^T_{t=1}$ without the need for region-specific gating networks. Then, pairwise relationships with both global and region-specific information are fused using Fusion module which encourages exploration without requiring an explicitly auxiliary loss. 


% \begin{equation}
% \begin{aligned}
% P^t_k &= \text{Softmax}\left(\left[-d(f^t_{k, \cdot}, f^i_{k, \cdot}) \right]_{i \in \{0, \ldots, T\} \setminus \{t\}}\right), \quad \forall k \in \{1, \cdots, H\}\\
% P^t &= \left[P^t_{1},\cdots, P^t_{H}\right]
% \end{aligned}
% \end{equation}


% \vspace{-1mm}
% \begin{equation}\label{eq:1}
% f_{\text{coo}}(\mathbf{x}^i) = \text{Fusion}(V(\mathbf{x}^i), P^i)
% % \vspace{-1mm}
% \end{equation}

% \textbf{Fusion.}\hspace{0.5mm} As shown in \textcolor{red}{Figure 3}, Fusion is a mechanism which can fusing a series of tensors of the same shape into one according to the given probability tensors. Fusion$(\cdot,\cdot)$ accept two parameters, in which the first is the list of tensors need to be fused, the second is the list of given probability tensors, each tensor and probability is of the same shape. During the training time, each element of the Fusion output is chosen by sampling from a Multinomial distribution whose probabilities and values are consists of the corresponding elements of each tensor in the given list of tensors and list of probability tensors, respectively. We can formulate this as:
% \begin{equation}
%     \boldsymbol{o}(i,j) = V_k(i,j),\ k \sim \text{Multinomial}(P_1(i,j),\cdots,P_K(i,j))
% \end{equation}
% in which $P = [P_1,\cdots,P_K]$, $V = [V_1,\cdots,V_K]$, $\boldsymbol{o} = \text{Fusion}(V,P)$, and here we assume each $V_k$ and $P_k$ is a 2D tensor for simplicity.
% When doing inference, Fusion calculates a corresponding expectation:
% \begin{equation}
%     \boldsymbol{o}(i,j) = \sum_{k=1}^{K}P_k(i,j)V_k(i,j)
% \end{equation}
% \textcolor{red}{According to our survey, the STAR module proposed in [SOFTs] appears to have done something similar. However, our Fusion mechanism is a superset of it since we decouple $P$ from $V$ so that $P$ can be given arbitrarily according to requirements.} From another perspective, Fusion can be seen as a kind of stochastic pooling which combines the advantages of max pooling and mean pooling. It can effectively improve the robustness and generalization of the model.


% Returning to the discussion of the pairwise cooperative item $f_{\text{coo}}(\mathbf{x}^i)$ in \eqref{eq:1}, in order to extract effective information from experts of other regions, intuitively the $V(\mathbf{x}^i)$ in \eqref{eq:1} should be:
% $$
% V(\mathbf{x}^i) = [f^0(\mathbf{x}^i),\cdots,\widehat{f^i(\mathbf{x}^i)},\cdots,f^N(\mathbf{x}^i)]
% $$
% where $\widehat{(\cdot)}$ means excluding this item from the sequence. However, when it comes to $P^i$, we need to decide to what extent the target region can refer to information from other regions. As we mentioned above, if two regions have similar load composition structures, then the way they use covariates to predict load will be similar to a certain extent. So we can use the performance of each expert to infer the similarity of each region and then determine the $P^i$. Concretely, we choose the $P^i$ as follow:
% $$
% P^i = \text{Softmax}([-d(f^i, f^0),\cdots,\widehat{-d(f^i,f^i)},\cdots,-d(f^i,f^N)])
% $$
% where $d(\cdot,\cdot)$ is the distance between two functions. Obviously, if two experts $f^i$ and $f^j$ are closer, they can refer to each other more when making predictions. Without loss of generality, we can assume each expert satisfies: $f^k \in L^1(\mathbb{R}^{(c-1)\times(L+P)+L}), \forall k=0,...,N $, and then we can choose  $d(f_1, f_2) = \int_{x\in D} |f_1(x)-f_2(x)|dx$. Note that each latent $f^j(\mathbf{x}^i) \in \mathbb{R}^{P \times d_{model}}$ in our setting, and we calculate each distance $d(f^i, f^j)$ in a dimension-wise way, therefore each distance keeps the same dimension: $d(f^i, f^j) \in \mathbb{R}^{P \times d_{model}}$. By this way, the relationship between two regions can be not unique, just as they may have similar industrial loads but very different living loads. 

% It is worth mentioning that calculating the integral requires traversing all samples in a region, which is impossible during training in a SGD way. So we calculate the integral using all samples in a batch instead. Besides, experts from other regions involved in the Fusion module only participates in forward calculations, but not in the back propagation of gradients so that training samples of one region would not affect the parameters of the expert of other regions. 
% \textcolor{red}{reason/reference to SOFTs.} We can formulate this as:
% % \vspace{-1mm}
% \begin{equation}\label{eq:fusion}
% \text{Fusion}(P, V) = \left\{
% \begin{aligned}
%      \text{Stoch\_Pool}(V), \quad \text{when training} \\
%      \mathbb{E}_P(V), \quad \text{when infering} \\
% \end{aligned}
% \right.
% % \vspace{-1mm}
% \end{equation}

% In conclusion, the output of the \textcolor{red}{RegionMixer} block $\mathbf{z}^i \in \mathbb{R}^{P\times 3d_{model}}$ can be formulated as:
% % \vspace{-1mm}\begin{align}\label{eq:conclusion}
% \begin{equation}
% \mathbf{z}^i = \text{CONCAT}(f^0(\mathbf{x}^i), f^i(\mathbf{x}^i), f_{coo}(\mathbf{x}^i))
% &f_{proximal}^i(\mathbf{x}^i) = \text{Fusion}(P, V) \nonumber\\
% &P = \text{Softmax}([-d(f_e^i,f_e^0),...,-d(f_e^i,f_e^{i-1}),-d(f_e^i,f_e^{i+1}),...,-d(f_e^i,f_e^N)]) \nonumber\\
% &V = [f_e^0(\mathbf{x}^i),...,f_e^{i-1}(\mathbf{x}^i),f_e^{i+1}(\mathbf{x}^i),...,f_e^N(\mathbf{x}^i)]
% &f_{proximal}^i = \sum_{j=0, j\neq i}^N \frac{exp(- d(f_e^i, f_e^j)}{\sum_{k=0, k\neq i}^N exp(-d(f_e^i, f_e^k)} \cdot f_e^j,  \\
% \vspace{-1mm}
% \end{equation}
% \textcolor{blue}{check the dimension of P.}
% where CONCAT$(\cdot)$ denote concatenating a series of tensors along the last dimension. Note that we also include general expert $f^0$ in Fusion mechanism, Therefore, even if there are no sufficiently similar regions to draw knowledge from, $f_{coo}$ will simply degenerate to general expert $f^0$ without causing negative migration from other regions.

% In \eqref{eq:encoder},  As for $f_{proximal}^i$, we can regard it as a function which captures the most similar load-covariates relationships between target city and other cities. In other words, we can \textcolor{red}{...}



 % Firstly we have to talk about why we need such a mechanism. 
 % As mentioned above, we can encode the global relationship among all cities through the general expert $f_e^0$ and encode specific relationship through city experts $f_e^i$. However, we are still missing some of the relationships shared by partial cities, which is exactly done by the Proximal Fusion $f_{proximal}^i$. As we see in \eqref{eq:encoder}, $f_{proximal}^i$ is the expectation of all experts's output of current sample except the target city-specific expert $f_e^i$, and the probabilities of the expectation is the Softmax of $-d(f_e^j, f_e^i), j = 0,...,i-1,i+1,...,N$, respectively. In this way, the Proximal fusion $f_{proximal}^i$ can extract information from other city experts according to the similarity of each two experts: $f_e^i$ and $f_e^j, j\neq i$. That is, for city $i$, we will calculate the distance of any other city expert $f_e^j$ with $f_e^i$, and use this distance as the degree of similarity between two cities. It is intuitive because if two cities have partially similar load-covariate relationships, then their experts' performance should be similar, too. For example, two coastal cities may both have a portion of the load associated with the port so that their load-covariates relationship show some degree of similarity. 


% It is worth mentioning that each expert is a high-dimensional function, i.e. $f_e : \mathbb{R}^{(c-1)\times(L+P)+L} \longmapsto \mathbb{R}^{P \times d}$. Therefore, we calculate $f_{proximal}^i$ in a dimension-wise way by which every dimension of $f_{proximal}^i$ can have different coefficient when calculating expectation. 


% f high-dimension, gradient bp, f integral imple

% We first introduce notations and outline the objective of LEAF. At each online forecasting period $p$, we have a training set $\mathcal{D}_{\mathrm{train}}^{p}= \left\{\mathbf{X}_{p}, \mathbf{Y}_{p} \right\}$ and a test set $\mathcal{D}_{\mathrm{test}}^{p}= \{ \Tilde{\mathbf{X}}_{p}, \Tilde{\mathbf{Y}}_{p} \}$.  Without loss of generality, we assume that both the training set and the test set contain $B$ samples. Specifically, $\mathbf{X}_{p} = \{ \mathbf{x}_{p}^{(i)} \}_{i=1}^{B}$ and $\Tilde{\mathbf{X}}_{p} = \{ \Tilde{\mathbf{x}}_{p}^{(i)} \}_{i=1}^{B}$. The main objective of LEAF is to leverage knowledge gained from historical periods and generate model parameters to make accurate forecasts on $\mathcal{D}_{\mathrm{test}}^{p}$ in the presence of concept drift. To achieve this goal, LEAF learns two functions: extrapolation $\mathcal{E}(\cdot;\boldsymbol{\phi}_{e})$ and adjustment $\mathcal{A}(\cdot;\boldsymbol{\phi}_{a})$, addressing macro- and micro-drift, respectively, to generate model parameters $\boldsymbol{\theta}_p$ at period $p$. The objective can be formulated as:
% % \vspace{-1mm}
% \begin{equation}
% \begin{aligned}
% &\mathop{\mathrm{min}}\limits_{\boldsymbol{\phi}_{e},\boldsymbol{\phi}_{a}} \, \sum_{i=1}^B \mathcal{L}(f(\Tilde{\mathbf{x}}_{p}^{(i)};\boldsymbol{\theta}_{p}^{(i)});\Tilde{\mathbf{y}}_{p}^{(i)}), \\ \quad \mathrm{s.t.,} \; \boldsymbol{\theta}_{p}^{(i)} &=\mathcal{A}(\boldsymbol{\theta}_{p},\Tilde{\mathbf{x}}_{p}^{(i)};\boldsymbol{\phi}_{a}), \; \boldsymbol{\theta}_{p}=\mathcal{E}(\boldsymbol{\theta}^*_{p-k:p-1};\boldsymbol{\phi}_{e}),
% \end{aligned}    
% % \vspace{-1mm}
% \end{equation}
% where the extrapolation function $\mathcal{E}(\cdot;\boldsymbol{\phi}_{e})$ is used to anticipate the macro-drift which takes as the optimal parameters $\boldsymbol{\theta}^*_{p-k:p-1}$ from the previous $k$ periods as input and infer parameters $\boldsymbol{\theta}_{p}$ for period $p$, the adjustment function performs sample-specific parameter adjustment considering micro-drift within each sample, and $\mathcal{L}(\cdot)$ is the prediction loss. Figure \ref{fig:leaf}(b) illustrates the framework of LEAF.
% \subsection{Model Overview.}

% Now we describe our proposed model at high level as shown in Figure \ref{fig:workflow}. Our model consists of a forecast model  $f_{\boldsymbol{\phi}_f}$, an extrapolation network $E_{\boldsymbol{\phi}_e}$, a latent decoder $D_{\boldsymbol{\phi}_d}$ and an adaptation module $M_{\phi_m}$. All the parameters $\boldsymbol{\phi} = \{\boldsymbol{\phi}_m, \boldsymbol{\phi}_f, \boldsymbol{\phi}_e, \boldsymbol{\phi}_d\}$ are first pre-trained on $\mathcal{D}^{warm}$, and the forecast model parameters $\boldsymbol{\phi}_f$ are fixed from now on. At each online step $k$, given a task instance $\mathcal{T}_k$, $H^*_k$ is obtained by differentiating $H$ w.r.t $\mathcal{L}^{\mathcal{D}^S_k}$ and a sequence of optimal latent codes $H^*_{k-n_h-1:k}$ from previous online steps which represents the evolving concept drift are encoded by $E_{\boldsymbol{\phi}_e}$ to extrapolate the latent code $H_k^Q$ for $\mathcal{D}^Q_k$. $H_k^Q$ captures the macro-drift in $\mathcal{D}^Q_k$ which can be interpreted as shared context for samples in  $\mathcal{D}^Q_k$. Afterwards, the covariates in query set $\{\mathcal{X}\}^{|\mathcal{D}^Q_k|}_{i=1}$ are encoded to hidden representation $\mathbf{z}$ by $g_{\boldsymbol{\phi}_g}$ and is adapted to $\mathbf{z}^\prime$ using ${M}_{\boldsymbol{\phi}_m}$ to cope with the covariates shift. The loss $\mathcal{L}^{\mathcal{D}^Q_k}$ is calculated and $\boldsymbol{\phi}_m, \boldsymbol{\phi}_e$ is updated  respectively using $\mathcal{L}^{\mathcal{D}^Q_k}$.

% We define the procedure that takes input lookback windows to $\mathbf{z}^\prime$ as the sample adaptation stage, and we define the procedure that extrapolates forecast model parameters as the extrapolation stage. 

% \begin{figure*}[!t]
% %\vspace{-5mm}
%     \centering
%     \includegraphics[width=1.0\textwidth]{figures/LEAF-framework.pdf}
%     \vspace{-7mm}
%     \caption{Model Architecture. (a) Warm-up of the target prediction model. The initial latent embedding $\boldsymbol{H}_{\mathrm{init}}$ is randomly generated and frozen during the warm-up phase, and the encoder is learned with prediction loss on warm-up dataset. (b) Meta-learning of LEAF which consists of three meta-learnable modules: extrapolation, adjustment, and parameter decoder.} 
%     \label{fig:leaf}
%     \vspace{-2mm}
% \end{figure*}



% \vspace{-2mm}
\subsubsection{CTSpecializer}
\label{section:CTSpecializer}
% \vspace{-2mm}
Following the stack of \(N_r\) RegionMixer layers, the representation \(\mathbf{X}^{t, N_r} \in \mathbb{R}^{H \times d_r}\) is obtained, encapsulating both region-specific and general information for region \(t\). The goal of the CTSpecializer is to further delineate the contextual and temporal variations. Let \(\mathbf{X}^{t, 0} = \mathbf{X}^{t, N_r}\) represent the starting latent representation for a stack of \(N_{l}\) CTSpecializer layers. As illustrated in Figure \ref{fig:model}, the process for any layer \(l \in \{1,\cdots, N_l\}\) is given by:
\begin{equation}
\begin{aligned}
\mathbf{X}^{t, l} = \text{CTSpecializer}(\mathbf{X}^{t, l-1}) + \mathbf{X}^{t, l-1}.
\end{aligned}
\end{equation}
CTSpecializer comprises two key components:
\begin{itemize}
    \item \textbf{Context-specializing MoE}. This component captures contextual variations between different instances, employing a set of experts \(\{g^{i, l}:  \mathbb{R}^{H \times d_r} \mapsto \mathbb{R}^{H \times d_r}\}^{N_c}_{i=1}\). These experts, implemented as multi-layer perceptrons (MLPs), operate on the latent dimension for each timestamp. For input \(\mathbf{X}^{t, l-1}\), the 3D probability tensor \(\mathbf{P}^{l} \in \mathbb{R}^{T \times H \times d_r}\) is constructed directly from expert activations \citep{han2024softs}, as follows:
    \begin{equation}  
    \mathbf{P}^{l}_{:,j,k} = \text{Softmax}\left( \left[g^{i, l}_{j, k} (\mathbf{X}^{t, l-1})\right]^{N_c}_{i=1} \right).
    \end{equation}  
    The Fusion module, as defined in Section \ref{section:regionmixer}, is applied to fuse the concatenated outputs of experts:
    \begin{equation}
    \mathbf{O}^l_{\text{cat}} = \{g^{i, l}(\mathbf{X}^{t,l})\}^{N_c}_{i=1} \in \mathbb{R}^{N_c \times H \times d_r},
    \end{equation} 
    with the input $\mathbf{X}^{t, l-1}$:
    \begin{equation}  
    \mathbf{\mathbf{X}}^{t, l} = \text{Fusion}\left(\mathbf{X}^{t, l-1},\mathbf{O}_{\text{cat}}, \mathbf{P}^{l}\right) \in \mathbb{R}^{H \times d_r}.
    \end{equation}  
    \item \textbf{Time-specializing MoE}. This component addresses temporal variations across instances. The output from context-specializing stage, \(\mathbf{X}^{t, l} \in \mathbb{R}^{H \times d_r}\), is transposed to \(\mathbf{X}^{t, l} \in \mathbb{R}^{d_r \times H}\) before being processed by a set of MLP experts \(\{h^{i, l}:  \mathbb{R}^{d_r \times H} \mapsto \mathbb{R}^{d_r \times H}\}^{N_t}_{i=1}\). A corresponding 3D probability tensor \(\mathbf{P}^{l} \in \mathbb{R}^{T \times d_r \times H}\) is similarly constructed from the resulting activations and the Fusion module is applied to fuse the outputs of experts with the input $\mathbf{X}^{t, l}$. The result is transposed back to \(\mathbf{X}^{t, l} \in \mathbb{R}^{H \times d_r}\).
\end{itemize}


% a set of experts $\{g^{c, l}_i:  \mathbb{R}^{H \times d_r} \mapsto \mathbb{R}^{H \times d_r}\}^{N_c}_{i=1}$ is used to capture contextual variations and another set of experts $\{g^{t, l}_i: \mathbb{R}^{H \times d_r} \mapsto \mathbb{R}^{H \times d_r}\}^{N_t}_{i=1}$ is used to capture temporal variations for all regions.
% The \textcolor{red}{RegionMixer} block can be viewed as a way to absorb differences between different regions by projecting the input variables of different regions into a common latent space where the latent representations of different regions can be treated in a unified way. This is exactly what we are going to implement in the next \textcolor{red}{CTSpecializer} block. As can be observed in \textcolor{red}{Figure 4(show GAM effect)}, when making predictions, samples of different weather conditions may have different activation levels for different covariates. For example, on a sunny day the temperature might be of more concern, on a cloudy day the humidity. Similarly, different weather conditions may also have different emphasis on features at different time points. Based on this, we designed two different dimensions of MoE in the \textcolor{red}{CTSpecializer} block, namely \textcolor{red}{CovariateMoE} and \textcolor{red}{TimeMoE}, as shown in \textcolor{red}{Figure 5}. Note that in our setting the \textcolor{red}{CTSpecializer} block can be stacked $L$ times.

% Concretely, the output of the \textcolor{red}{RegionMixer} is first processed by \textcolor{red}{CovariateMoE} layer, which consists of $E$ covariate experts. Here $E$ is a hyper parameter means the number of experts in \textcolor{red}{CTSpecializer} block. Each covariate expert is a 2-layer MLP along the covariate dimension. The $E$ outputs of these experts can be denoted as:
% $$
% g_l^e(\mathbf{z}_{l-1}) \in \mathbb{R}^{P \times d_{model}}, \quad e \in \{1,\cdots,E\}
% $$
% where $\mathbf{z}_l$ represents the output of the $l^{\text{th}}$ \textcolor{red}{CTSpecializer} block and $\mathbf{z}_0$ is the output of the \textcolor{red}{RegionMixer} block. To fuse $E$ experts' output, we do not use the common gating mechanism in MoE. Instead, we use the Fusion mechanism proposed in \ref{section:citymoe} as following way:
% \begin{equation}
%     \tilde{\mathbf{z}_l} = \text{Fusion}(\text{Softmax}(\tilde{V}(\mathbf{z}_{l-1})), \tilde{V}(\mathbf{z}_{l-1}))
% \end{equation}
% where $\tilde{V}(\mathbf{z}_{l-1}) = [g_l^1(\mathbf{z}_{l-1}),...,g_l^E(\mathbf{z}_{l-1})]$. Here we set the probability in Fusion mechanism simply by normalizing the softmax activations of the output of $E$ experts. To some extent, this can be seen as a stochastic pooling of $E$ experts, which is a combination of max pooling and average pooling.

% Almost identical to CovariateMoE, the TimeMoE layer does the same thing along the time dimension. Denoting the $E$ experts of the TimeMoE layer as $h_l^1,\cdots,h_l^E$, we can formulate the output of TimeMoE as:
% \begin{equation}
%     \mathbf{z}_l = \text{Fusion}(\text{Softmax}(V(\tilde{\mathbf{z}_l})), V(\tilde{\mathbf{z}_l}))
% \end{equation}
% where $V(\tilde{\mathbf{z}_l}) =[h_l^1(\tilde{\mathbf{z}_l}),...,h_l^E(\tilde{\mathbf{z}_l})]$. It is worth mentioning that there exist a residual connection between any two adjacent TimeMoE layer and CovariateMoE layer.
% As shown in \textcolor{red}{Figure 4}, after projecting the input tensor to the common latent space, the following processing procedures can be regarded as the same for each city. That is to say, we put the city-related parts mainly in the CityMoE block, and in the latent space we believe that the latent representations of different cities can be processed in a unified way. We design a WeaMoE block to better process the latent representation to higher level. 

% As we can see, WeaMoE contains two types of experts of orthogonal dimensions which work in turn. One group of experts is responsible for handling the relationship in the time dimension, and the other is responsible for the covariate dimension. 

In traditional manual forecasting methods, a historical interval of length $H$ is initially selected based on its contextual similarity to the future forecast horizon. The forecast is then constructed by examining the differences in covariate values between this historical interval and the intended forecast horizon. Drawing inspiration from this approach, we encourage contextually similar samples to be processed by similar context-specializing experts. This is achieved through the integration of a contrastive loss, which encourages the model to differentiate between varying contexts by reinforcing similarities and distinctions among the samples. Specifically, for each raw training sample \(\mathbf{X}_n^t\) from region \(t\), a positive sample \(\overline{\mathbf{X}}_n^t\) and a set of negative samples \(\{\widetilde{\mathbf{X}}_i^t\}_{i=1}^{N_n}\) are generated. These samples are differentiated based on the Euclidean distances computed across salient covariates such as weather conditions, electricity pricing, and date. In any CTSpecializer layer \(l \in \{1, \cdots, N_l\}\), the context-specialized outputs for the primary training sample, its positive, and negative counterparts are denoted as \(\mathbf{X}_n^{t, l}\), \(\overline{\mathbf{X}}_n^{t, l}\), and \(\{\widetilde{\mathbf{X}}_i^{t, l}\}_{i=1}^{N_n}\), respectively. The contrastive loss for the training sample \(n\) is expressed as:

\begin{equation} 
l^{t}_{n} = -\frac{\exp\left(\text{sim}(\mathbf{X}_n^{t, l}, \overline{\mathbf{X}}_n^{t, l}) / \tau\right)}{\exp\left(\text{sim}(\mathbf{X}_n^{t, l}, \overline{\mathbf{X}}_n^{t, l}) / \tau\right) + \sum^{N_n}_{i=1}\exp\left(\text{sim}(\mathbf{X}_n^{t, l}, \widetilde{\mathbf{X}}_n^{t, l}) / \tau\right)},
\end{equation}  
where $\tau$ is the temperature parameter \citep{chen2020simple} and the similarity $\text{sim}(\mathbf{U}, \mathbf{V})$ between two matrices $\mathbf{U}, \mathbf{V} \in \mathbb{R}^{H \times d_r}$ is calculated by first flatten matrices into vectors and apply cosine similarities between two vectors using dot product and $l_2$ norm,  formulated as:
\begin{equation} 
\begin{aligned}
\mathbf{u} &= \text{Flatten}(\mathbf{U})\in \mathbb{R}^{(H \times d_r)},\\
\mathbf{v} &= \text{Flatten}(\mathbf{V}) \in \mathbb{R}^{(H \times d_r)},\\
\text{sim}(\mathbf{\mathbf{u}}, \mathbf{v}) &= \frac{\mathbf{u} \cdot \mathbf{v}}{\|\mathbf{u}\|\|\mathbf{v}\|}.
\end{aligned}
\end{equation}  

\subsubsection{Loss function} For a region \(t\) with a mini-batch \(\{\mathbf{X}^t_n\}_{n=1}^N\), after processing through \(N_r\) RegionMixer layers and \(N_l\) CTSpecializer layers, predictions are generated using a region-specific projection head \(\phi_t: \mathbb{R}^{H \times d_r} \rightarrow \mathbb{R}^{H \times 1}\):
\begin{equation} 
\mathbf{\hat{y}}_n = \phi_t(\mathbf{X}^{t, N_l}_n).
\end{equation}  
The complete loss function integrates both the mean squared error (MSE) loss and the contrastive loss, defined as follows:
\begin{equation} 
\mathcal{L} = \frac{1}{N}\sum_{t=1}^{T}\sum_{i=1}^{N} (\mathbf{\hat{y}}_i - \mathbf{y}_i)^2 + \alpha \cdot l^t_{i}, 
\end{equation}  
where \(\alpha\) denotes the regularization parameter balancing the contributions between the MSE and contrastive losses.
% In order to encourage similar samples to be processed by the same experts and to better exert the ability of MoE, we design a contrast loss for each TimeMoE layer and CovariateMoE layer.
% In addition, the WeaMoE layer also introduces a contrastive learning mechanism so that similar weather conditions are processed by the same expert, which effectively distinguishes each expert, with different experts responsible for processing samples of different classes. 

% To be specific, we can denote $E, g_l, h_l$ the number of experts in WeaMoE block, the time expert and the covariate expert respectively, we can formulate the WeaMoE block as follow:
% \vspace{-1mm}
% \begin{equation}\label{eq:weamoe}
% \begin{aligned}
% &P = \text{Softmax}([h_l^1(\hat{\mathbf{z}_l}),...,h_l^E(\hat{\mathbf{z}_l})])
% % &f_{proximal}^i = \sum_{j=0, j\neq i}^N \frac{exp(- d(f_e^i, f_e^j)}{\sum_{k=0, k\neq i}^N exp(-d(f_e^i, f_e^k)} \cdot f_e^j,  \\
% \end{aligned}
% % \vspace{-1mm}
% \end{equation}


% \textbf{TimeMoE.}\hspace{0.5mm} We use $E$ time experts to encode the relationship along the time dimension of latent representation. For example, one expert may focus on the morning, while other expert focus more on afternoon. For Simplicity, each time expert is chosen as a two-layer MLP:
% $$
% g_l^m(\mathbf{z}) = (\text{MLP}(\mathbf{z}^T))^T.
% $$
% where $\mathbf{z} \in \mathbb{R}^{P\times d_{model}}$ is latent representation of some layer, $m \in \{1,...,E\}$.  
% Combined with the contrastive learning that will be mentioned later, 

% \textbf{CovariateMoE.}\hspace{0.5mm} Correspondingly, there are $E$ covariate experts doing the same thing along the covariate dimension.
% $$
% h_l^m(\hat{\mathbf{z}}) = \text{MLP}(\hat{\mathbf{z}}).
% $$
% CovariateMoE uses the same Fusion mechanism as TimeMoE. As shown in \eqref{eq:weamoe}, TimeMoE and CovariateMoE execute alternatively layer by layer. 
% In addition, combined with the contrastive learning that will be mentioned later, both of the TimeMoE and CovariateMoE layer can activate the same expert when encounter the similar input, Which further promotes the division of labor among different experts.
% For each layer of the WeaMoE block, we add a contrastive loss to promote each expert in a layer to focus on one kind of similar days. For example, one expert deals with rainy day while another handles sunny day.
% \textbf{Contrastive loss.}\hspace{0.5mm} We denote $gh^e(\cdot), \ e \in \{1,\cdots,E\}$ the TimeMoE layer or the CovariateMoE layer in any CTSpecializer block. For every input sample $\mathbf{x}$, we first find the most similar sample $\mathbf{x}^+$ and the least similar sample $\mathbf{x}^-$ of it. Note that we use the size of the value output by each expert as the relative size of its probability of being selected in these layers. So we need to make the probability for selecting experts of positive samples closer and the probability of negative samples farther away. To achieve this, we add the following cosine similarity loss item:
% \begin{equation}
% \begin{aligned}
%     l_1 = -\sum_{i,j}\frac{P(\mathbf{z})[i,j]\cdot P(\mathbf{z}^+)[i,j]}{||P(\mathbf{z})[i,j]||\cdot||P(\mathbf{z}^+)[i,j]||} \\
%     + \sum_{i,j}\frac{P(\mathbf{z})[i,j]\cdot P(\mathbf{z}^-)[i,j]}{||P(\mathbf{z})[i,j]||\cdot||P(\mathbf{z}^-)[i,j]||}
%     \end{aligned}
% \end{equation}
% where $P(\cdot)[i,j] = \text{Softmax}(gh^1(\cdot)[i,j],\cdots,gh^E(\cdot)[i,j])$ and $\mathbf{z}$, $\mathbf{z}^+$, $\mathbf{z}^- $ are the input of this layer, which are the latent of $\mathbf{x}$, $\mathbf{x}^+$, $\mathbf{x}^- $, respectively.

% On the other hand, we also need the final output of each TimeMoE layer or CovariateMoE layer to be as close as possible for each pair of similar samples, where final output means the Fusion output of the experts of this layer. We just need an InfoNEC loss to do this:   
% % \vspace{-1mm}
% \begin{equation}\label{eq:contraloss}
% l_2 = - \log \frac{\exp(\text{sim}(\boldsymbol{o}(\mathbf{z}), \boldsymbol{o}(\mathbf{z}^+)))}{\exp(\text{sim}(\boldsymbol{o}(\mathbf{z}), \boldsymbol{o}(\mathbf{z}^+))) + \exp(\text{sim}(\boldsymbol{o}(\mathbf{z}), \boldsymbol{o}(\mathbf{z}^-)))} 
% % \vspace{-1mm}
% \end{equation}
% where $\boldsymbol{o}(\cdot)[i,j] = P(\cdot)[i,j] \cdot V(\cdot)[i,j]$ and  $V(\cdot)[i,j] = (gh^1(\cdot)[i,j],\\ \cdots,gh^E(\cdot)[i,j])$. Finally, the contrastive loss can be formulated as:
% $$
% l_{\text{contra}} = \alpha \cdot l_1 + \beta \cdot l_2
% $$
% where $l_1$ loss is supposed to make the similar samples activate the same expert as much as possible, and $l_2$ loss aims at making the MoE block's outputs more similar when dealing with the positive samples. 
% During the extrapolation stage, the meta-model LEAF aims at inferring a prediction model based on previously optimal models. It focuses on generating overall suitable model parameters for the next period by tracking and anticipating the macro-drift between different periods of data. However, we have observed that although LEAF is used to generate a bulk of model parameters, it does not need to operate on high-dimensional parameter spaces. This is because model parameters are used to depict complex data patterns, most of which remain invariant, and only a small part will experience drift. In other words, the concept drift can be effectively modeled in a low-dimensional latent space. As a result, we introduce a latent embedding $\boldsymbol{H}$ which can be decoded to the model parameter $\boldsymbol{\theta}$
% % (the detailed training procedure of the decoder is described in Section \ref{section:model_learning})
% , and the extrapolation is performed on this latent space.

% In period $p$, we have $\mathcal{D}_{\mathrm{train}}^{p}= \left\{\mathbf{X}_{p}, \mathbf{Y}_{p} \right\}$ and  $\mathcal{D}_{\mathrm{test}}^{p}= \{ \Tilde{\mathbf{X}}_{p}, \Tilde{\mathbf{Y}}_{p} \}$. In particular, $\mathcal{D}_{\mathrm{train}}^{p}$ is identical to the test data $\mathcal{D}_{\mathrm{test}}^{p-1}$, as shown in Figure \ref{fig:online_time_series_forecasting}. In other words, if we optimize the prediction model on $\mathcal{D}_{\mathrm{train}}^{p}$, we can obtain the optimal model at period $p-1$ in the latent space as follows:
% \begin{equation}
%   \boldsymbol{H}^*_{p-1} = \mathrm{SGD}(\boldsymbol{H}_{p-1},\mathcal{L}^{\mathrm{train}},\mathcal{D}_{\mathrm{train}}^{p}),
% \end{equation}
% where $\mathrm{SGD}$ represents gradient descent on $\mathcal{D}_{\mathrm{train}}^{p}$ with respect to prediction loss. This optimization process leads to the optimal latent embedding $\boldsymbol{H}^*_{p-1}$. Subsequently, we introduce an extrapolation network $\mathrm{NN}(\cdot)$ that infers $\boldsymbol{H}_{p}$ based on the previous $k$ optimal latent embeddings $\boldsymbol{H}^*_{p-k:p-1}$ and a decoder to generate model parameters, which can be formulated as:
% \begin{equation}
% \begin{aligned}
%       \boldsymbol{H}_{p} = \mathrm{NN}(\boldsymbol{H}^*_{p-k:p-1}),   \quad    \boldsymbol{\theta}_{p} = \mathrm{Decoder}(\boldsymbol{H}_{p}).
% \end{aligned}
% \label{eq:LSTM}
% \end{equation}
% Moving forward period $p+1$, $\mathcal{D}_{\mathrm{test}}^{p}$ (or $\mathcal{D}_{\mathrm{train}}^{p+1}$) is revealed. The above steps can be repeated to obtain $\boldsymbol{H}^*_{p}$, $\boldsymbol{H}_{p+1}$ and $\boldsymbol{\theta}_{p+1} $. $\mathrm{NN}(\cdot)$ can be any sequential model, e.g., LSTM and Transformer. We utilize a simple LSTM here as default to verify the capability of the framework itself. Besides, we investigate the network selection of the extrapolation network (see Appendix \ref{appendix:sensitiviy}).

% % \begin{figure*}[!t]
% % % \vspace{-10mm}
% %     \centering
% %     \includegraphics[width=0.8\linewidth]{figures/LEAF-framework-yf.pdf}
% %     % \vspace{-3mm}
% %     \caption{Model Architecture. (a) Warm-up of the target prediction model. The initial latent embedding $\boldsymbol{H}_{\mathrm{init}}$ is randomly generated and frozen during the warm-up phase, and the encoder is learned with prediction loss on warm-up dataset. (b) Meta-learning of LEAF which consists of three meta-learnable modules: extrapolation, adjustment, and parameter decoder.} 
% %     \label{fig:leaf}
% %     % \vspace{-4mm}
% % \end{figure*}

% % Given a task instance $\mathcal{T}_k$, the goal of this stage is to extrapolate the hidden code $H^Q_k$ using a sequence of optimal latent codes $\{H^*_{1:k-1}\}$ that represent historical data distributions. that will fit well on the query set $\mathcal{D}^Q_k$. []  The overall procedure is shown in Eq. \ref{eq:extrapolation}. First, a sequence of $(H^*_{})$ for $\mathcal{D}^S_{k}$ is first optimized for several gradient steps using SGD to obtain the latent representation $H^*_k$ of $\mathcal{D}^S_{k}$, then a sequence of latent representations of past datasets are encoded to extrapolate the latent code for $\mathcal{D}^Q_{k}$ using latent encoder $E_{\boldsymbol{\phi}_e}$. Lastly, the parameters $\boldsymbol{\phi}^Q_f$ for query set $\mathcal{D}^Q_{k}$ is decoded using latent decoder $D_{\boldsymbol{\phi}_d}$. 

% % \begin{gather}\label{eq:extrapolation}
% % H^*_k = SGD(\alpha, H^Q_{k-1}, \mathcal{L}^{\mathcal{D}^S_k}) \\
% % H^* = [H^*_{k-n_h-1}, H^*_{k-1}, ...., H^*_k]\\
% % H^Q_k = E_{\boldsymbol{\phi}_e} (H^*)\\
% % \boldsymbol{\phi}^Q_f = D_{\boldsymbol{\phi}_d}(H^Q_k)
% % \end{gather}

% % \vspace{-2mm}
% \subsubsection{Learning to Adjust via Surrogate Loss}
% \label{section:adjustment}
% % \vspace{-2mm}
% The inferred model in the extrapolation stage is designed to anticipate and account for macro-drift. However, they do not consider the micro-drift that can occur within each individual sample. 
% As the historical and forecast horizon of time series tend to coexist within an identical domain, it is quite beneficial to perform model adaptation to capture the micro-drift at inference (test) time according to the input $\Tilde{\mathbf{X}}$.
% % {\color{blue}During the period of influence, the unlabeled $\Tilde{\mathbf{X}}$ encapsulates substantial information pertinent to the distributions of the test data. This is particularly salient in the domain of time series forecasting, where the input and output variables coexist within an identical domain and exhibit strong correlations. Recent advancements in methodology have given rise to the concept of test-time training ~\citep{sun2020test}, which involves the application of a self-supervised loss function during the testing phase to accommodate shifts in the distribution of individual data samples. Nonetheless, the process of identifying an efficacious self-supervised auxiliary task or an unsupervised loss function presents considerable challenges in the context of time series forecasting, given the phenomenon of concept drift. The scarcity of research in this area and the inherent heterogeneity of time series datasets—where a self-supervised auxiliary task may prove effective for traffic time series but fail to generalize to financial time series—further complicates this endeavor.} 
% To this end, we introduce a meta-learnable surrogate loss that adjusts or modulates the latent embedding $\boldsymbol{H}_{p}$ for each sample $\{ \Tilde{\mathbf{x}}_{p}^{(i)} \}_{i=1}^{B}$ in $\mathcal{D}_{\mathrm{test}}^{p}$ to obtain sample-specific embeddings $\{ \boldsymbol{H}_{p}^{(i)} \}_{i=1}^{B}$. This surrogate loss is implemented using neural networks and applied during the testing phase, enabling the adjustment of the latent embedding based on sample-specific characteristics.

% The rationale behind this approach is that micro-drift is often caused by external events, such as weather conditions or holidays. Although data affected by micro-drift may exhibit different patterns, they tend to deviate from their context in a similar manner. For example, the electricity consumption pattern during the summer typically differs from that in the winter, while during holidays it tends to decrease regardless of the season. 
% % The electricity consumption pattern during the summer typically differs from that in the winter. In the summer, due to factors such as increased use of air conditioning, electricity consumption tends to be higher compared to the winter season. However, during holidays, regardless of the season, electricity consumption tends to decrease. This is because many businesses and households reduce their energy usage during holiday periods when there is less demand for electricity.
% By incorporating a meta-learnable surrogate loss, we aim to capture and adjust for these sample-specific deviations caused by micro-drift. Specifically, during the meta-training phase, the surrogate loss is learned to capture and compensate for different types of deviations. During the meta-testing phase, the model utilizes the learned surrogate loss to adjust the latent embedding based on the specific characteristics of each individual sample. To achieve this, the loss network takes into account the following three factors to capture sample-specific micro-drift:

% %\vspace{-1mm}
% \textbf{Sample and base prediction.}\hspace{0.5mm}The sample itself $\Tilde{\mathbf{x}}_{p}^{(i)}$ and the base prediction with inferred model parameters in extrapolation stage $f(\Tilde{\mathbf{x}}_{p}^{(i)};\boldsymbol{\theta}_{p})$ are introduced as basic characteristics.

% %\vspace{-1mm}
% \textbf{Base latent embedding.}\hspace{0.5mm} Another important part of information is the prediction model. As we optimize the model in a latent space, the inferred latent embedding in the extrapolation stage $\boldsymbol{H}_{p}$ is passed to the loss network, providing the contextual information and underlying pattern. 

% % \vspace{-1mm}
% \textbf{Sample's relationship to training data.}\hspace{0.5mm} Furthermore, we introduce a relation network to account for sample's relationship to its context. The relation network $\mathcal{R}(\cdot)$ receives embeddings of the sample $\Tilde{\mathbf{x}}_{p}^{(i)}$ and training set $\mathcal{D}_{\mathrm{train}}^{p}$ and returns a vector representing their relationship:
% \begin{equation}
%     \boldsymbol{R}_{p}^{(i)} = \mathcal{R} \left( g(\Tilde{\mathbf{x}}_{p}^{(i)}), {\mathbb{E}}_{ {\mathbf{x}}_{p}^{(j)} \sim \mathcal{D}_{\mathrm{train}}^{p} } g( {\mathbf{x}}_{p}^{(j)} ) \right),
% \end{equation}
% where $g(\cdot)$ is an embedding function, and the training data embedding is computed as the mean pooling of embeddings of all samples in the training set. The relation network captures the similarities or dissimilarities in their patterns, which is valuable in capturing the micro-drift. 
% To sum up, the final loss network $s(\cdot)$ are defined as
% %%takes these features as input and returns a scalar value as the surrogate loss:
% \begin{equation}
% \label{equ:surrogate_loss}
% \mathcal{L}^{\mathrm{surrogate}}(\Tilde{\mathbf{x}}_{p}^{(i)}) = s \left(\Tilde{\mathbf{x}}_{p}^{(i)},f(\Tilde{\mathbf{x}}_{p}^{(i)};\boldsymbol{\theta}_{p}),\boldsymbol{H}_{p},\boldsymbol{R}_{p}^{(i)} \right).
% \end{equation}
% The surrogate loss guides the adjustment of the latent embedding for each sample using gradient descent, which can be further decoded to obtain sample-specific model parameters:
% % \vspace{-2mm}
% \begin{equation}
% \begin{aligned}
%       \boldsymbol{H}_{p}^{(i)} = \boldsymbol{H}_{p} - \alpha \nabla_{\boldsymbol{H}_{p}} \mathcal{L}^{\mathrm{surrogate}}(\Tilde{\mathbf{x}}_{p}^{(i)}), \quad \boldsymbol{\theta}_{p}^{(i)}  = \mathrm{Decoder}(\boldsymbol{H}_{p}^{(i)}),
% \end{aligned}
% % \vspace{-2mm}
% \end{equation}

% where $\alpha$ is the learning rate, and $\boldsymbol{H}_{p}^{(i)}$ and $\boldsymbol{\theta}_{p}^{(i)}$ stand for sample-specific latent embedding and model parameters, respectively. Finally, the parameters are loaded to make forecasts with $f(\Tilde{\mathbf{x}}_{p}^{(i)});\boldsymbol{\theta}_{p}^{(i)})$.

% % The surrogate loss are generated introduces these features to generate

% % To cope with the covariates shift, given a task instance $\mathcal{T}_k$, the goal is to find a self-supervised loss function $\mathcal{L}_{self}$ such that make one gradient step on the input hidden representation w.r.t the loss will facilitate forecasts on $\mathcal{D}^Q_{k}$. Instead of an explicit self-supervised loss [BYOL, SimCLR], we propose to learn an implicit dynamic self-supervised loss function using meta-learning [MLLN]. 
% % \begin{gather}\label{eq:extrapolation}
% % \mathbf{z} = g_{\boldsymbol{\phi}_g} (\mathcal{X}^Q) \\
% % \mathbf{z}^\prime  \leftarrow \mathbf{z} -\beta\nabla_{\mathbf{z}} \mathcal{L}_{self} (\mathbf{z}, \mathcal{M}(\mathbf{z})) 
% % \end{gather}
% % \begin{equation}
% %     \boldsymbol{H}_p^{(i)} = g
% % \end{equation}

% \begin{algorithm}[t]
%     % \scriptsize
%     \small
%     \SetAlgoLined
%     \KwIn{Number of meta-training periods $P$, data $\{ \mathcal{D}_{\mathrm{train}}^{p}, \mathcal{D}_{\mathrm{test}}^{p}\}_{p=1}^P$, learning rates $\eta$, $\alpha$, $\mu$, number of historical periods in extrapolation stage $k$, prediction model $f(\cdot)$}
%     % \KwResult{Output result}
%     \BlankLine

%     Randomly initialize the parameters $\boldsymbol{\phi}_e $, $\boldsymbol{\phi}_a$, and $\boldsymbol{\omega}$ of LEAF  \;
%     Let $\boldsymbol{\psi} = \{ \boldsymbol{\phi}_e, \boldsymbol{\phi}_a, \boldsymbol{\omega} \}$ \;
%     Randomly initialize the latent embedding $\boldsymbol{H}_{0}$ \;
%     Create a queue $\mathcal{Q}$ of size $k$ storing the recent $k$ optimal latent embeddings\;
%     Initialize $\mathcal{Q}$ as $\mathcal{Q} = [\boldsymbol{H}_{0}, \cdots,\boldsymbol{H}_{0} ]$ \;

		
%     \For{$ p = 1, 2, \cdots, P $}{
%         Evaluate inner-loop prediction loss  $\mathcal{L}_{p}^{\mathrm{train}}$ on training dataset $\mathcal{D}_{\mathrm{train}}^{p}$ ;

%         Perform gradient descent $\boldsymbol{H}_{p-1}^* = \boldsymbol{H}_{p-1} - \eta \nabla_{\boldsymbol{H}_{p-1}}\mathcal{L}_{p}^{\mathrm{train}}$;

%         % (f_{\boldsymbol{\theta}_{p-1}})

%         $\mathcal{Q}.\mathrm{Deque}().\mathrm{Enque}(\boldsymbol{H}_{p-1}^*.\mathrm{detach}())$
        
%         Compute $\boldsymbol{H}_{p}$ and $\boldsymbol{\theta}_{p}$ using Equation (\ref{eq:LSTM}); \quad {\color{black}/* Extrapolation stage */}
        
%         \For{$ \Tilde{\mathbf{x}}_{p}^{(i)} $ in $\Tilde{\mathbf{X}}_{p}$ }{

%              {\color{black}/* Adjustment stage: traverse all test inputs, and conduct sample-specific adjustment */}
            
%             Compute $\mathcal{L}^{\mathrm{surrogate}}(\Tilde{\mathbf{x}}_{p}^{(i)})$ using Equation (\ref{equ:surrogate_loss});

%             $\boldsymbol{H}_{p}^{(i)} = \boldsymbol{H}_{p} - \alpha \nabla_{\boldsymbol{H}_{p}} \mathcal{L}^{\mathrm{surrogate}}(\Tilde{\mathbf{x}}_{p}^{(i)})$;
            
%             $\boldsymbol{\theta}_{p}^{(i)}  = \mathrm{Decoder}(\boldsymbol{H}_{p}^{(i)})$, and load  $\boldsymbol{\theta}_{p}^{(i)}$ into $f(\cdot)$;

%             Evaluate  prediction loss  $\mathcal{L}_{p,i}^{\mathrm{test}}$ w.r.t. $ \Tilde{\mathbf{x}}_{p}^{(i)} $ ;
%         }

%         Compute $\mathcal{L}^{\mathrm{LEAF}}$ using Equation (\ref{eq:outer_loop});
        
%         Perform gradient descent $\boldsymbol{\psi} = \boldsymbol{\psi} - \mu \nabla_{\boldsymbol{\psi}} \mathcal{L}^{\mathrm{LEAF}} $;
%     }
%     \caption{Training Procedure of LEAF}
%     \label{algo:training}
% \end{algorithm}

% % \vspace{-2mm}
% \subsubsection{Model Learning}\label{section:model_learning}
% % \vspace{-2mm}
% In this subsection, we outline the training procedure of LEAF, as depicted in Algorithm \ref{algo:training}. We denote the parameters of extrapolation module and adjustment module as $\boldsymbol{\phi}_e $ and $\boldsymbol{\phi}_a$, respectively. Additionally, $\boldsymbol{\omega}$ represents the parameter of the decoder. 

% At each period $p$, as shown in Figure \ref{fig:leaf}(b), after extrapolation and adjustment stages (the ``inner loop"), we make predictions on $\mathcal{D}^p_{\text{test}}$. The test set is then utilized to update the parameters of meta-learners $\boldsymbol{\phi}_a$, $\boldsymbol{\phi}_e$, $\boldsymbol{\omega}$ (the "outer loop"). More precisely, the optimization process of "outer loop" is performed by minimizing the following objective:
% \begin{equation} \label{eq:outer_loop}
% \footnotesize
% \begin{aligned}
%  \mathcal{L}^{\mathrm{LEAF}} = \mathop{\mathrm{min}}\limits_{\boldsymbol{\phi}_{e},\boldsymbol{\phi}_{a}, \boldsymbol{\omega}} \, \sum_{i=1}^B\mathcal{L}^{\mathrm{test}}(f(\Tilde{\mathbf{x}}_{p}^{(i)};\boldsymbol{\theta}_{p}^{(i)});\Tilde{\mathbf{y}}_{p}^{(i)}) 
%  + \gamma \|\mathrm{stopgrad}(\boldsymbol{H}^*_p) - \boldsymbol{H}_p\|^2_2,   
% \end{aligned}
% \end{equation}
% where the first term is the prediction loss on the test set, the second term regularizes the extrapolation in Equation (\ref{eq:LSTM}) to output latent embedding that is close to the optimal latent embedding, and $\gamma$ is the coefficient of the regularization.

% Recall that online forecasting often involves a warm-up phase. Since we optimize the parameters of the prediction model in the latent space, the traditional training strategy is not directly applicable. To address this issue, we randomly generate a latent embedding $\boldsymbol{H}_{\mathrm{init}}$, which is then decoded into parameters of prediction model using the decoder. During the training procedure of the warm-up phase,  $\boldsymbol{H}_{\mathrm{init}}$ remains fixed and the decoder is trained using the prediction loss on warm-up dataset. Subsequently, at the onset of the meta-learning, we initialize $\boldsymbol{H}_{0}$ with $\boldsymbol{H}_{\mathrm{init}}$ and $\boldsymbol{\omega}$ with the learned decoder parameter from warm-up phase. Figure \ref{fig:leaf}(a) illustrates the warm-up strategy. 

% %%%{\color{blue} 
% \textbf{Remarks.} \hspace{1mm} LEAF generates the parameters for the last few layers of the target prediction model. It is important to note that LEAF is a model-agnostic framework, allowing different types of layers. For instance, when using DLinear as the target prediction model, we could generate the parameters for the linear layer. In the case of PatchTST, we could generate the parameters for the last transformer block, which includes the Query/Key/Value projection networks and a feed-forward network. To apply LEAF to different types of layers, we require the parameter shapes of the network layers. By flattening the parameters to be generated, we can determine the width of the decoder in LEAF. The generated parameters are then appropriately reshaped and loaded into the respective layers, allowing for flexibility and compatibility across different network architectures.
% %%%}
% % \vspace{-3mm}
% \subsection{Theoretical Analysis}
% % \vspace{-2mm}
% %%% three % denotes the original text in the revision.
% %%%In this section, we provide a theoretical analysis to underpin our proposed framework--learning to extrapolate and adjust. During each online forecasting period $p$, the dataset $\left\{\mathbf{X}_{p}, \mathbf{Y}_{p} \right\}$ is drawn from $\mathcal{P}_p$, where $\mathbf{X}_{p} = \{ \boldsymbol{x}_{p}^{(i)} \}_{i=1}^{B}$, $\mathbf{Y}_{p} = \{ \boldsymbol{y}_{p}^{(i)} \}_{i=1}^{B}$, and $B$ denotes the number of samples. Define that feature-target pair  $\boldsymbol{z} = [\boldsymbol{x};\boldsymbol{y}]$. A linear model $\hat{\boldsymbol{y}} = \mathbf{W}\boldsymbol{x}$ is adopted for the forecasting task. Assuming that we need to forecast at the current period $P+1$, with optimal parameters obtained from the preceding periods, our objective is to learn weights $\mathbf{W}_{P+1}$ that deliver robust generalization at period $P+1$. We posit two mild while reasonable assumptions regarding the concept drift within the data:

% In this section, we provide a theoretical analysis to underpin our proposed framework. During each online forecasting period $p$, the dataset $\left\{\mathbf{X}_{p}, \mathbf{Y}_{p} \right\}$ is drawn from $\mathcal{P}_p$, where $\mathbf{X}_{p} = \{ \boldsymbol{x}_{p}^{(i)} \}_{i=1}^{B}$, $\mathbf{Y}_{p} = \{ \boldsymbol{y}_{p}^{(i)} \}_{i=1}^{B}$, and $B$ denotes the number of samples. Define that feature-target pair  $\boldsymbol{z} = [\boldsymbol{x};\boldsymbol{y}]$. To simplify the discussion, in this analysis we assume a linear model $\hat{\boldsymbol{y}} = \mathbf{W}\boldsymbol{x}$ for the forecasting task. Assuming that we need to forecast at the current period $P+1$, with optimal parameters obtained from the preceding periods, our objective is to learn weights $\mathbf{W}_{P+1}$ that deliver robust generalization at period $P+1$. We introduce two mild conditions to characterize two different drifts. 

% \begin{assump}[Macro-drift] \small
% $\mathcal{P}_{p+1}$, the data distribution for period $P+1$, is a composite of $\mathcal{P}_{p}$ and an unknown distribution  $\mathcal{P}_{\Delta}$ that accounts for macro-drift and is independent of $\mathcal{P}_{p}$.
% \end{assump}

% \begin{assump}[Micro-drift] \small
% A transformed sample $\boldsymbol{z}^{\prime} = f(\boldsymbol{z}, \mathcal{P}) + \epsilon$ embodies micro-drift, and $f(\boldsymbol{z},\mathcal{P})= \boldsymbol{z} + \alpha\boldsymbol{\Sigma}^{-\frac{1}{2}}(\boldsymbol{z}-\boldsymbol{\mu})$  is a deterministic function with unknown scalar $\alpha$ responsible for the incremental change within each sample considering its distribution context.  
% $\boldsymbol{\mu}$ and $\boldsymbol{\Sigma}$ stand for mean and covariance of $\mathcal{P}$. $\epsilon $ follows a normal distribution $\mathcal{N}(0,\mathrm{diag}(\boldsymbol{\sigma}^2))$ denoting the stochastic noise. We denote this data distribution as $\mathcal{P}'$.
% \end{assump}

% Then we formulate two propositions to justify the methodology for learning the weights of the linear model to ensure accurate forecasting at period $P+1$ under concept drifts.

% \begin{prop}\label{prop:extrapolation1}\small
%     Given the complete datasets from preceding periods $\left\{\mathbf{X}_{p}, \mathbf{Y}_{p} \right\}_{p=1}^P$, the associated optimal weights $\left\{ \mathbf{W}_p^* \right\}_{p=1}^P$ and the input data $\left\{\mathbf{X}_{P+1} \right\}$ for period $P+1$. We approximate  weights for period $P+1$ as
%     \begin{equation}
%     \begin{aligned}
%         &\hat{\mathbf{W}}_{P+1} =  (\mathbf{X}^{\top}_{P+1}\mathbf{X}_{P+1})^{-1}(\mathbf{X}^{\top}_{P}\mathbf{X}_{P}\mathbf{W}^*_{P} + \hat{\mathbf{A}}), \text{s.t.} \nonumber\\
%         &\hat{\mathbf{A}} = \operatorname*{argmin}_{\mathbf{A}} \sum_{p=1}^{P-1} \left\|\mathbf{X}^{\top}_{p}\mathbf{X}_{p}\mathbf{W}^*_{p} + \mathbf{A} - \mathbf{X}^{\top}_{p+1}\mathbf{X}_{p+1}\mathbf{W}^*_{p+1} \right\|_{\mathrm{F}}^2. \nonumber
%     \end{aligned}
%     \end{equation}
%     This estimation exhibits much more generalization than the estimation with the last period:
%     \begin{equation*}        \mathbb{E}_{\mathcal{P}_{p+1}}\left\|\boldsymbol{y}- \hat{\mathbf{W}}_{P+1}\boldsymbol{x}\right\|^2 \ll \mathbb{E}_{\mathcal{P}_{p+1}}\left\|\boldsymbol{y}- \mathbf{W}^*_{P}\boldsymbol{x}\right\|^2.
%     \end{equation*}    
% \end{prop}
% % \vspace{-3mm}

% Note that the optimization of $\mathbf{A}$ in this proposition essentially seeks an optimal additive matrix to extrapolate the weights $\mathbf{W}^*_{p}$ to the subsequent period. Thereafter, we can deduce $\mathbf{W}^*_{P+1}$ by extrapolation from  $\mathbf{W}^*_{P}$  using this additive matrix. The proof is provided in the Appendix \ref{appendix:thereo}. Moreover, we establish the generalization error bound of this estimation and demonstrate that it is substantially superior to conventional fine-tuning approaches. Proposition \ref{prop:extrapolation1} highlights the significance of model extrapolation to achieve robust generalization performance under concept drifts. 

% %%%{\color{red}As we encounter increasingly intricate data scenarios and models, it becomes imperative to devise more sophisticated methods of model extrapolation.}

% \begin{prop}\label{prop:adjustment}\small
%     Considering the micro-drift, We possess the dataset $\left\{\mathbf{X}'_{p}, \mathbf{Y}'_{p} \right\}_{p=1}^P$, the associated optimal weights $\left\{ \mathbf{W}_p^* \right\}_{p=1}^P$ and the input data $\left\{\mathbf{X}'_{P+1} \right\}$ for period $P+1$. A sample-level weight adjustment achieves less prediction error than weight estimation in Proposition 1:
%       \begin{equation*}
%       \footnotesize
%       \begin{aligned}
%         &\mathbb{E}_{\mathcal{P'}_{p+1}}\left\|\boldsymbol{y}'- (\hat{\mathbf{W}}_{P+1}+\mathbf{\Psi})\boldsymbol{x}'\right\|^2 <
%         \mathbb{E}_{\mathcal{P'}_{p+1}}\left\|\boldsymbol{y}'- \hat{\mathbf{W}}_{P+1}\boldsymbol{x}'\right\|^2, \\
%         &\mathbf{\Psi}=\mathbf{\Sigma}'_{P+1,xx}^{-\frac{1}{2}}(\boldsymbol{x}'-\boldsymbol{\mu}'_{P+1,x})(\boldsymbol{x}'-\boldsymbol{\mu}'_{P+1,x})^{\top}\mathbf{\Sigma}'_{P+1,xx}^{-\frac{1}{2}}\mathbf{X}'_{P+1}^{\top}\mathbf{X}_{P+1}'\hat{\mathbf{W}}_{P+1},
%       \end{aligned}
%     \end{equation*}
%     where $\boldsymbol{\mu}_x$ and $\mathbf{\Sigma}'_{xx}$ are the mean and covariance of $\mathbf{X'}_{P+1}$, respectively.
% \end{prop}
% % \vspace{-3mm}

% Proposition 2 states that introducing a sample-dependent weight modification can alleviate the micro-drift. It implies that performing the sample-specific weight adjustment can reduce the prediction error in the context of sample-level micro-drift.

% Although our theoretical framework focuses on simplified linear models, the insights are highly relevant to real-world applications. This relevance is underscored by the fact that in numerous practical scenarios, only the parameters in the final linear layer of deep neural networks are updated, aligning with our theoretical approach. Moreover, even for nonlinear layers, practical evidence supports the effectiveness of our extrapolation and adjustment principles. To illustrate this, we conducted experiments applying LEAF solely to the last linear layer of a complex deep model where the assumptions of the above theoretical analysis tend to hold. The findings, presented in Table \ref{table:linear or nonlinear}, confirm that focusing LEAF on just the final linear layer yields benefits comparable to its application across multiple layers.

% % As for micro-drift, although we only consider a linear transformation of  sample in Assumption 2, the data distribution actually evolve non-linearly. As a result, only linear extrapolation of weights in Proposition \ref{prop:extrapolation} can no longer account for the micro-drift
